SemRe-Rank: Improving Automatic Term Extraction By Incorporating Semantic Relatedness With Personalised PageRank

Automatic Term Extraction deals with the extraction of terminology from a domain specific corpus, and has long been an established research area in data and knowledge acquisition. ATE remains a challenging task as it is known that there is no existing ATE methods that can consistently outperform others in any domain. This work adopts a refreshed perspective to this problem: instead of searching for such a 'one-size-fit-all' solution that may never exist, we propose to develop generic methods to 'enhance' existing ATE methods. We introduce SemRe-Rank, the first method based on this principle, to incorporate semantic relatedness - an often overlooked venue - into an existing ATE method to further improve its performance. SemRe-Rank incorporates word embeddings into a personalised PageRank process to compute 'semantic importance' scores for candidate terms from a graph of semantically related words (nodes), which are then used to revise the scores of candidate terms computed by a base ATE algorithm. Extensively evaluated with 13 state-of-the-art base ATE methods on four datasets of diverse nature, it is shown to have achieved widespread improvement over all base methods and across all datasets, with up to 15 percentage points when measured by the Precision in the top ranked K candidate terms (the average for a set of K's), or up to 28 percentage points in F1 measured at a K that equals to the expected real terms in the candidates (F1 in short). Compared to an alternative approach built on the well-known TextRank algorithm, SemRe-Rank can potentially outperform by up to 8 points in Precision at top K, or up to 17 points in F1.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex 


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf


==> figures/UNUSED-figure_ssr_avgP_z=100.tex <==
\begin{figure}[ht!]
  \centering
    \includegraphics[width=153mm]{figures/ssr_avgP_z=100.png}    
      \caption{Comparing SemRe-Rank against Adp-TextRank by \textbf{the improvement in average P@K} over base ATE methods for all five $k$'s considered.See Figure \ref{ssr_avgP_z=200} caption for how to interpret results on this Figure. (This figure is best viewed in colour) }\label{ssr_avgP_z=100}
\end{figure}

==> figures/UNUSED-figure_ssr_f1_z=100.tex <==
\begin{figure}[ht!]
  \centering
    \includegraphics[width=153mm]{figures/ssr_f1_z=100.png}    
      \caption{Comparing SemRe-Rank against Adp-TextRank by \textbf{the improvement in F1@RTP} over base ATE methods. See Figure \ref{ssr_avgP_z=200} caption for how to interpret results on this Figure.  (This figure is best viewed in colour) }\label{ssr_f1_z=100}
\end{figure}

==> figures/UNUSED-figure_ussr_avgP_z=100.tex <==
\begin{figure}[ht!]
  \centering
    \includegraphics[width=153mm]{figures/ussr_avgP_z=100.png}    
      \caption{Improvements in average P@K over base ATE methods by the unsupervised variant of SemRe-Rank. See Figure \ref{ssr_avgP_z=200} caption for how to interpret results on this Figure. (This figure is best viewed in colour) }\label{ussr_avgP_z=100}
\end{figure}

==> figures/UNUSED_figure_ussr_f1_z=100.tex <==
\begin{figure}[ht!]
  \centering
    \includegraphics[width=153mm]{figures/ussr_f1_z=100.png}    
      \caption{Improvements in F1@RTP by the unsupervised variant of SemRe-Rank  over base ATE methods. See Figure \ref{ssr_avgP_z=200} caption for how to interpret results on this Figure.  (This figure is best viewed in colour) }\label{ussr_f1_z=100}
\end{figure}

==> tables/TODO-tab_result_adp-textrank_z=100,200.tex <==
\begin{table*}[t!]
\centering
\small
\caption{(TODO: THIS TABLE HAS NOT BEEN UPDATED. SEE CHART_data.xlsx, chart-avgP and chart-F1@RTP worksheets for details)Full results of Adp-TextRank (using the same seed term sets for personalisation) against each base ATE method. Only the changes over the base ATE methods are shown as points within a scale of [0, 1], and (brackets) indicate negative changes. }\label{tab_result_adp-textrank} 
\resizebox{150mm}{!}{
\begin{tabular}{|l |l |l |l|l |l|l|l|l|l|l|l|l|l|l|}
\hline
Metric     	&\rotatebox[origin=c]{270}{Basic}	&\rotatebox[origin=c]{270}{\shortstack{Combo\\Basic}}		&\rotatebox[origin=c]{270}{LP}				&\rotatebox[origin=c]{270}{NTM}	&\rotatebox[origin=c]{270}{PU}	&\rotatebox[origin=c]{270}{Vote\textsubscript{5}}			&\rotatebox[origin=c]{270}{CValue}	  &\rotatebox[origin=c]{270}{\shortstack{Gloss-\\Ex}} 	&\rotatebox[origin=c]{270}{RAKE}	&\rotatebox[origin=c]{270}{\shortstack{Rele-\\vance}}	&\rotatebox[origin=c]{270}{TFIDF}	&\rotatebox[origin=c]{270}{\shortstack{Weird-\\ness}}	&\rotatebox[origin=c]{270}{$\chi^{2}$}	&\rotatebox[origin=c]{270}{Vote\textsubscript{7}}\\
\hline
\multicolumn{15}{|c|}{ACLv2}\\
\hline
$z$=100 P@K CNGs  	&\textbf{4}	&3		&3		&2			&\textbf{5}	 &\textbf{4}	&4				&\textbf{5}	&5		&5				&\textbf{4}		&4		&5}		&4\\
$z$=200 P@K CNGs  	&1			&3		&3		&4}		&4		&3		&4		&4		&5		&5		&3		&4		&3		&4\\

$z$=100 avg P@K		&.014}		&.01	&.018			&.01	&.032}	&.01}	&.022}	&.01		&.092			&.126}	&.058}	&.022			&.042}	&.026}\\
$z$=200 avg P@K	&.01				&.01	&.022}	&.01	&.018			&.004			&.004			&.01		&.098}	&.086			&.01			&.03}	&.018			&.016\\
%z=500 avgP@K	    &.02}	&.013}	&.003}	&.01	&.02}	&.02}	&.01}	&.08}	&.09}	&.02}	&.04}	&.03}\\
\hline

$z$=100 P@RTP   &-		&-		&-	&-		&-				&-		&.01}	&.01	&.03}		&.01			&.01}		&-	&.01	&.01\\
$z$=200 P@RTP    	&-		&-	&-	&-		&-		&-	&-	&.01	&.02	&.01	&-		&-	&.01	&.01\\
$z$=100 R@RTP   &.003	&-		&-	&.04	&.01}	&-		&.002}	&.01	&.04}		&.03}	&.01}		&-	&.01	&.002\\
$z$=200 R@RTP    	&.003	&-	&-	&.04	&.005	&-	&-	&.01	&.02	&.02	&.002	&-	&.01	&.002\\
$z$=100 F1@RTP  &-		&-		&-	&.02	&.003}	&-		&.01}	&.01	&.03}		&.02}	&.01}		&-	&.01	&.01\\
$z$=200 F1@RTP   	&-		&-	&-	&.02	&.002	&-	&-	&.01	&.02	&.01	&-		&-	&.01	&.01\\
%z=500 diff ovrl P)    	&.01	&-		&-	&.02	&-				&.01	&.01	&.02			&.02	&	-				&-	&-\\
%z=500 diff ovrl R)    	&.01	&.002}	&-	&.02	&.005}	&.01	&.01	&.02			&.03	&	-				&.001}	&-\\
%z=500 diff ovrl F1)   	&.01	&-		&-	&.02	&.002}	&.01	&.01	&.021}	&.03	&	-				&-	&-\\
\hline
\multicolumn{15}{|c|}{GENIA}\\
\hline
$z$=100 P@K CNGs  	&4		&4		&4			&5}		&2				&5		&5				&4		&5				&5				&4}		&5		&5		&3\\
$z$=200 P@K CNGs  	&4		&4		&5}		&4		&2		&5		&5		&4		&5		&5		&3		&5		&5		&4}\\

$z$=100 avg P@K		&.01			&.01			&.038			&.01	&.036}	&.01	&.014	&.04	&.062}	&.106}	&.03}	&.078}	&.026}	&.01}\\
$z$=200 avg P@K	&.012}	&.012}	&.044}	&.01	&.01			&.01	&.014	&.04	&.058			&.104			&.018			&.076			&.022			&.004\\

%z=500 avgP@K	    &.02}	&.02}	&.04	&.013}	&.02	&.012}	&.04}	&.06}	&.12}	&.033}	&.08	&.022}\\
\hline
$z$=100 P@RTP    	&.01			&-	&-	&-	&-	&-		&.02}	&-		&.03	&-				&.04	&.01	&.01	&.01\\
$z$=200 P@RTP    	&.01	&-	&-	&-	&-	&-		&.01	&-		&.03	&-	&.04	&.01	&.01	&.01\\
$z$=100 R@RTP    	&.01}	&-	&-&-	&-	&.004	&.02}	&.007	&.04	&-				&.04	&.01	&.01	&.01}\\
$z$=200 R@RTP    	&.002	&-	&-	&-	&-	&.004	&.01	&.007	&.04	&-	&.04	&.01	&.01	&.004\\
$z$=100 F1@RTP   	&.01	&-	&-	&-	&-	&-				&.02}	&.003	&.04	&-				&.04	&.01	&.01	&.01\\
$z$=200 F1@RTP   	&.01	&-	&-	&-	&-	&-		&.01	&.003	&.04	&-	&.04	&.01	&.01	&.01\\
%z=500 diff ovrl P)    	&.01	&-	&-0.02	&-	&-		&.01	&-		&.02	&.01	&.04	&.01	&.01\\
%z=500 diff ovrl R)    	&.012}	&-	&-0.02	&-	&-		&.01	&.007}	&.03	&.01	&.03	&.01	&.01\\
%z=500 diff ovrl F1)   	&.011}	&-	&-0.02	&-	&-		&.01	&.003}	&.03	&.01	&.04	&.01	&.01\\
\hline
\multicolumn{15}{|c|}{TTCm}\\
\hline
$z$=100 P@K CNGs  	&4	&4}	&1}	&5}	&2}	&4}	&3	&3	&3}	&5	&4	&5	&3	&4}\\
$z$=200 P@K CNGs  		&4		&2		&-		&2		&1		&3		&3		&4}			&2		&5		&4		&5		&3		&3\\
$z$=100 avg P@K	    &.01	&.01}	&.004}	&.02}	&.03}	&.01}	&.068}	&.01}	&.01	&.126}	&.068}	&.05}	&.08}	&.022}\\
$z$=200 avg P@K	&.01	&.004			&-				&.01			&(.01)			&.004	&.01	&-							&.01	&.104	&.028	&.044	&.01	&.01\\

%z=500 avgP@K	    &.02}	&.02}	&.01}	&-	&-	&.03}	&0.01	&.01}	&.03}	&-0.01}	&.01}	&-0.03\\
\hline
$z$=100 P@RTP    	&-	&-	&-	&.05}	&.01}	&.02}		&-	&.01}	&.01}	&.14}	&.03}	&.08}	&.01	&.02}\\
$z$=200 P@RTP    	&-		&-		&-		&.02	&-	&-		&-		&-		&-		&.08	&.02	&.04	&.01	&-\\
$z$=100 R@RTP    	&-	&-	&.01	&.08}	&.01}	&.02}		&.01	&.01}	&.03}	&.21}	&.06}	&.11}	&.03	&.05}\\
$z$=200 R@RTP    	&-		&-		&.01	&.04	&-	&-		&.01	&.004	&.01	&.16	&.04	&.05	&.03	&.01\\
$z$=100 F1@RTP   	&-	&-	&-	&.06}	&.01}	&.02}		&.002	&.01}	&.01}	&.17}	&.04}	&.09}	&.02	&.03}\\
$z$=200 F1@RTP   	&-		&-		&-		&.03	&-	&-		&.002	&-		&-		&.12	&.03	&.04	&.02	&.003\\

%z=500 diff ovrl P)    	&-	&-	&-	&.02}	&-		&-0.01	&-	&-	&-}	&-}	&.03}	&-}\\
%z=500 diff ovrl R)    	&-	&-	&-	&.03}	&.005}		&-0.02	&-	&.01}	&.01}	&-}	&.04}	&-}\\
%z=500 diff ovrl F1)   	&-	&-	&-	&.02}	&.002}		&-0.01	&-	&-	&.004}	&-}	&.03}	&-}\\
\hline
\multicolumn{15}{|c|}{TTCw}\\
\hline
$z$=100 P@K CNGs  	&2	&2	&1}	&3}	&2}	&2}	&2}	&2}	&-	&5}	&4}	&5}	&4}	&3\\
$z$=200 P@K CNGs	&2			&2		&-	&2		&1			&1		&1		&-	&-	&5		&3		&3		&2		&3\\
$z$=100 avg P@K	    &.01}	&.01}	&.004}	&.032}	&.042}	&.01	&.012}	&.01}	&-	&.096}	&.046}	&.026}	&.022}	&.022}\\
$z$=200 avg P@K	   	&(.006)	&-	&-	&.01	&(.01)	&.01	&.01	&-	&-	&.054	&.012	&.014	&.01	&.01\\


%z=500 avgP@K	    &-0.01	&-0.01	&-0.01	&-	&-0.01	&.01	&-0.01	&-	&.02	&-	&.01	&-\\
\hline
$z$=100 P@RTP    	&-	&-		&-	&.03}	&-	&.01}		&.02}		&-	&-	&.10}	&.02}	&.04}	&.02}	&.01}\\
$z$=200 P@RTP    	&.01		&-			&-		&.01		&-			&-		&.01	&-	&-	&.08	&.01	&.02	&-		&-\\
$z$=100 R@RTP    	&.03}	&.03}	&.02}	&.05}	&-	&.02}		&.04}	&-	&-	&.17}	&.05}	&.06}	&.05}	&.01}\\
$z$=200 R@RTP    	&(.01)		&.004		&-		&.01		&-			&-		&.01	&-	&-	&.14	&.03	&.03	&-		&-\\
$z$=100 F1@RTP   	&.01}	&.01}	&-	&.04}	&-	&.01}		&.03}	&-	&-	&.13}	&.05}	&.05}	&.03}	&.01}\\
$z$=200 F1@RTP   	&(.01)		&-			&-		&.01		&-			&-		&.01	&-	&-	&.10	&.02	&.03	&-		&-\\
%z=500 diff ovrl P)    	&-	&-		&-	&-	&-		&-		&-	&-	&-	&-0.01	&.01	&-\\
%z=500 diff ovrl R)    	&-	&.01	&-	&-	&-		&.01	&-	&-	&-	&-0.03	&.01	&-\\
%z=500 diff ovrl F1)   	&-	&.003	&-	&-	&-		&.003	&-	&-	&-	&-0.02	&.01	&-\\
\hline
\end{tabular}
}
\end{table*}



==> tables/tab_dataset_expanded.tex <==
\begin{table}[t!]
\centering
\small
\caption{Statistics of the expanded datasets (indicated by the \textit{dbp} subscript) following the described method. \#docs - number of documents in the dataset; \#words - number of words (using white space as separator), without any filtering such as stop words removal. This also includes duplicates.}\label{tab_dataset_expanded} 
\begin{tabular}{l | l |l |l |l |l}
\hline
		   &	    &\multicolumn{4}{c}{\#words in docs} \\\cline{3-6}
Dataset    &\#docs	&total 	&min	&mean	&max \\
\hline
GENIA\textsubscript{dbp}     &3,452  &2,348,394	&5	&680	&13,804\\
ACLv2\textsubscript{dbp}	    &452	&368,071	&10		&814	&9,488\\
TTCw\textsubscript{dbp}  	&1,400	&4,211,348	&9	&3,008	&67,088\\
TTCm\textsubscript{dbp} 		&1,173		&3,185,324	&14	&2,715	&54,727\\
\hline
\end{tabular}
\end{table}



==> tables/tab_dc.tex <==
\begin{table}[t!]
\centering
\small
\caption{Results of Domain Coherence (DC) obtained on the four datasets.}\label{tab_dc} 
\begin{tabular}{l | l |l |l |l |l|l|l|l}
\hline
	&\multicolumn{5}{c|}{P@K} &\multicolumn{3}{c}{PRF1@RTP}\\
\hline
	&50	&100	&500 	&1000	&2000	&P	&R	&F1\\
\hline
ACLv2     	&.72  &.72 	&.58	&.48	&.38	&.37	&.46	&.41\\
GENIA     	&.80  &.77 	&.63	&.56	&.52	&.33	&.44	&.38\\
TTCm     	&.34  &.41 	&.19	&.11	&.06	&.29	&.50	&.37\\
TTCw     	&.44  &.32 	&.14	&.09	&.05	&.20	&.36	&.26\\
\hline
\end{tabular}
\end{table}


==> tables/tab_dc_changes.tex <==
\begin{table}[t!]
\centering
\small
\caption{Results of applying SemRe-Rank (SSR) and its unsupervised variant (uSSR) to DC on the four datasets. Only the changes to the base DC results are shown. (Brackets) indicate decreases. The average P@K (avg P@K) figures are calculated as average over the five different $K$'s, including also the $K$'s where no changes are noticed.}\label{tab_dc_changes} 
\begin{tabular}{l | l |l |l |l |l}
\hline
DC with...			&P@K CNGs	&avg P@K	&P@RTP 	&R@RTP	&F1@RTP\\
\hline
\multicolumn{6}{c}{ACLv2}\\
\hline
SSR, $z=100$     	&4  &(.004) 	&(.03)	&(.03)	&(.03)\\
uSSR, $z=100$     	&5  &(.014)	 	&(.03)	&(.03)	&(.03)\\
SSR, $z=200$     	&4  &(.01) 		&(.03)	&(.04)	&(.03)\\
uSSR, $z=200$     	&5  &(.018) 	&(.03)	&(.04)	&(.03)\\
\hline
\multicolumn{6}{c}{GENIA}\\
\hline
%DC with...			&P@K CNGs	&avg P@K	&P@RTP 	&R@RTP	&F1@RTP\\\hline
SSR, $z=100$     	&2  &.006 	&(.02)	&(.02)	&(.02)\\
uSSR, $z=100$     	&3  &- 		&(.02)	&(.02)	&(.02)\\
SSR, $z=200$     	&2  &.006 	&(.01)	&(.01)	&(.01)\\
uSSR, $z=200$     	&2  &.002 	&(.02)	&(.02)	&(.02)\\
\hline
\multicolumn{6}{c}{TTCm}\\
\hline
%DC with...			&P@K CNGs	&avg P@K	&P@RTP 	&R@RTP	&F1@RTP\\\hline
SSR, $z=100$     	&2  &(.01) 		&(.01)	&(.02)	&(.01)\\
uSSR, $z=100$     	&3  &(.004) 	&(.03)	&(.05)	&(.04)\\
SSR, $z=200$     	&1  &(.024) 	&-		&(.01)	&(.002)\\
uSSR, $z=200$     	&3  &(.002) 	&(.04)	&(.06)	&(.05)\\
\hline
\multicolumn{6}{c}{TTCw}\\
\hline
%DC with...			&P@K CNGs	&avg P@K	&P@RTP 	&R@RTP	&F1@RTP\\\hline
SSR, $z=100$     	&3  &.02 	&-	&-	&-\\
uSSR, $z=100$     	&0  &- 	&-	&-	&-\\
SSR, $z=200$     	&3  &.016 	&-	&-	&-\\
uSSR, $z=200$     	&0  &- 	&-	&-	&-\\
\hline
\end{tabular}
\end{table}


==> tables/tab_graph_stats.tex <==
\begin{table}[t!]
\centering
\small
\caption{Statistics of constructed graphs on the four datasets. \textit{avg\#nodes}: average number of nodes per document; \textit{avg\#edges}: average number of undirected edges per document; \textit{\%connected G}: \% of documents that has a single connected graph. %We also show the average active elements in the personalization vector (Equation \ref{e_ppagerank}) per document under different $m$.}\label{tab_graph_stats} 
}\label{tab_graph_stats}
\begin{tabular}{l | l |l |l |l}
\hline
		   &ACLv2	    &GENIA	&TTCm	&TTCw\\
\hline
avg\#nodes     	&525  	&2,023	&5,793		&8,813\\
avg\#edges	    &1,976	&5,028	&254,236	&165,669\\
\%connected G  	&94\%	&96\%	&72\%		&67\%\\
\hline
%\multicolumn{5}{c}{vector initialization}\\
%\hline
%m=100 		&88		&23	&94			&74\\
%m=200 		&159	&36	&190		&147\\
%m=500 		&315	&104	&-	&-\\
%\hline
\end{tabular}
\end{table}



==> tables/tab_graph_stats_supervised.tex <==
\begin{table}[t!]
\centering
\small
\caption{Statistics of vector initialization with filtered terms (supervised SemRe-Rank). Other graph stats (e.g., nodes, edges) remain the same as those in Table \ref{tab_graph_stats}.}\label{tab_graph_stats_supervised} 
\begin{tabular}{l | l |l |l |l}
\hline
		   &ACLv2	    &GENIA	&TTCm	&TTCw\\
%\hline
%avg\#nodes     	&854  	&5,000	&11,499		&24,401\\
%avg\#edges	    &3,147	&11,549	&458,693	&479,891\\
%\%connected G  	&94\%	&97\%	&69\%		&73\%\\
%\hline
%\multicolumn{5}{c}{personalized TermRank vector initialization}\\
\hline
m=100 		&64		&17	&32		&23\\
m=200 		&111	&27	&50		&39\\
%m=500 		&315	&104	&-	&-\\
\hline
\end{tabular}
\end{table}



==> tables/tab_graph_stats_supervised_tr.tex <==
\begin{table}[t!]
\centering
\small
\caption{Statistics of vector initialization with filtered terms (supervised SemRe-Rank). Other graph stats (e.g., nodes, edges) remain the same as those in Table \ref{tab_graph_stats}.}\label{tab_graph_stats_supervised} 
\begin{tabular}{l | l |l |l |l}
\hline
		   &ACLv2	    &GENIA	&TTCm	&TTCw\\
%\hline
%avg\#nodes     	&854  	&5,000	&11,499		&24,401\\
%avg\#edges	    &3,147	&11,549	&458,693	&479,891\\
%\%connected G  	&94\%	&97\%	&69\%		&73\%\\
%\hline
%\multicolumn{5}{c}{personalized TermRank vector initialization}\\
\hline
m=100 		&62		&16	&31		&11\\
m=200 		&101	&25	&63		&19\\
%m=500 		&315	&104	&-	&-\\
\hline
\end{tabular}
\end{table}



==> tables/tab_graph_stats_wd.tex <==
\begin{table}[t!]
\centering
\small
\caption{Statistics of constructed graphs on the four datasets. \textit{avg\#nodes}: average number of nodes per document; \textit{avg\#edges}: average number of undirected edges per document; \textit{\%connected G}: \% of documents that has a single connected graph. We also show the average active elements in the personalization vector (Equation \ref{e_ppagerank}) per document under different $m$.}\label{tab_graph_stats} 
\begin{tabular}{l | l |l |l |l}
\hline
		   &ACLv2	    &GENIA	&TTCm	&TTCw\\
\hline
avg\#nodes     	&854  	&5,000	&11,499		&24,401\\
avg\#edges	    &3,147	&11,549	&458,693	&479,891\\
\%connected G  	&94\%	&97\%	&69\%		&73\%\\
\hline
\multicolumn{5}{c}{vector initialization}\\
\hline
m=100 		&90		&26	&95			&78\\
m=200 		&167	&43	&191		&156\\
%m=500 		&315	&104	&-	&-\\
\hline
\end{tabular}
\end{table}



==> tables/tab_kcr.tex <==
\begin{table}[t!]
\centering
\small
\caption{Results of KeyConceptRelatedness (KCR) obtained on the four datasets.}\label{tab_kcr} 
\begin{tabular}{l | l |l |l |l |l|l|l|l}
\hline
	&\multicolumn{5}{c|}{P@K} &\multicolumn{3}{c}{PRF1@RTP}\\
\hline
	&50	&100	&500 	&1000	&2000	&P	&R	&F1\\
\hline
ACLv2     	&.78  &.73 	&.60	&.51	&.36	&.36	&.44	&.40\\
GENIA     	&.92  &.92 	&.71	&.68	&.65	&.31	&.39	&.35\\
TTCm     	&.42  &.29 	&.12	&.08	&.05	&.21	&.34	&.26\\
TTCw     	&.38  &.32 	&.11	&.07	&.04	&.19	&.34	&.24\\
\hline
\end{tabular}
\end{table}


==> tables/tab_kcr_changes.tex <==
\begin{table}[t!]
\centering
\small
\caption{Results of applying SemRe-Rank (SSR) and its unsupervised variant (uSSR) to KCR on the four datasets. Only the changes to the base KCR results are shown. (Brackets) indicate decreases. The average P@K (avg P@K) figures are calculated as average over the five different $K$'s, including also the $K$'s where no changes are noticed.}\label{tab_kcr_changes} 
\begin{tabular}{l | l |l |l |l |l}
\hline
KCR with...				&P@K CNGs	&avg P@K	&P@RTP 	&R@RTP	&F1@RTP\\
\hline
\multicolumn{6}{c}{ACLv2}\\
\hline
SSR, $z=100$     	&3  &.062 	&-	&-	&-\\
uSSR, $z=100$     	&4  &.022 	&-	&-	&-\\
SSR, $z=200$     	&4  &.06 	&-	&-	&-\\
uSSR, $z=200$     	&4  &.01 	&-	&-	&-\\
\hline
\multicolumn{6}{c}{GENIA}\\
\hline
SSR, $z=100$     	&4  &(.032) 	&-	&-	&-\\
uSSR, $z=100$     	&4  &(.030)		&-	&-	&-\\
SSR, $z=200$     	&5  &(.032) 	&-	&-	&-\\
uSSR, $z=200$     	&4  &(.028) 	&-	&-	&-\\
\hline
\multicolumn{6}{c}{TTCm}\\
\hline
SSR, $z=100$     	&2  &(.034) &(.02)	&-	&(.02)\\
uSSR, $z=100$     	&4  &.052 	&-		&.04	&.01\\
SSR, $z=200$     	&4  &.02 	&(.01)	&.005	&(.06)\\
uSSR, $z=200$     	&4  &.10 	&.08	&.17	&.11\\
\hline
\multicolumn{6}{c}{TTCw}\\
\hline
SSR, $z=100$     	&3  &.016 	&-	&.01	&.003\\
uSSR, $z=100$     	&2  &.05 	&-		&.02	&.004\\
SSR, $z=200$     	&1  &.016 	&-	&.03	&.01\\
uSSR, $z=200$     	&3  &.056 	&.02	&.06	&.03\\
\hline
\end{tabular}
\end{table}


==> tables/tab_result_changes.tex <==
\begin{table*}[t!]
\centering
\small
\caption{Numbers of $P@K$s where changes are noticed when compared against each baseline ATE method.}\label{tab_result_changes} 
\begin{tabular}{|l |l |l |l |l||l|l|l|l|l|l|l|}
\hline
					&\multicolumn{4}{l||}{ATR4S} 	&\multicolumn{7}{l|}{JATE}\\
\hline
     	&\shortstack{Combo\\Basic}	&LP	&NTM	&PU	&CValue	  &\shortstack{Gloss-\\Ex} 	&RAKE	&\shortstack{Rele-\\vance}	&TFIDF	&\shortstack{Weird-\\ness}	&$\chi^{2}$\\
\hline
\multicolumn{12}{|c|}{ACLv2}\\
\hline
TermRankStd	    			&3	&2	&2	&4	&2	&4	&5	&5	&2	&4	&3\\
\hline
TermRankPsn m=100 (P)    	&3	&3	&5	&4	&5	&4	&5	&5	&3	&4	&4\\
TermRankPsn m=200 (R)    	&3	&3	&5	&4	&3	&5	&5	&5	&2	&4	&3\\
%TermRankPsn m=500 (F1)   	&3	&3	&3	&3	&1	&4	&5	&5	&3	&4	&2\\
\hline
\multicolumn{12}{|c|}{GENIA}\\
\hline
TermRankStd	    			&5	&5	&5	&2	&4	&4	&5	&5	&3	&5	&5\\
\hline
TermRankPsn m=100 (P)    	&4	&4	&4	&1	&5	&4	&5	&5	&3	&5	&5\\
TermRankPsn m=200 (R)    	&4	&5	&5	&2	&5	&4	&5	&5	&3	&5	&5\\
%TermRankPsn m=500 (F1)   	&4	&5	&4	&2	&5	&4	&5	&5	&3	&5	&5\\
\hline
\multicolumn{12}{|c|}{TTCm}\\
\hline
TermRankStd	    			&1	&0	&1	&1	&1	&0	&0	&3	&3	&2	&1\\
\hline
TermRankPsn m=100 (P)    	&3	&1	&3	&1	&2	&2	&2	&5	&4	&5	&3\\
TermRankPsn m=200 (R)    	&2	&1	&1	&1	&3	&1	&2	&5	&3	&4	&3\\
\hline
\multicolumn{12}{|c|}{TTCw}\\
\hline
TermRankStd	    			&1	&1	&3	&1	&1	&0	&0	&3	&0	&2	&0\\
\hline
TermRankPsn m=100 (P)    	&2	&0	&2	&1	&2	&1	&0	&5	&3	&4	&3\\
TermRankPsn m=200 (R)    	&2	&0	&2	&1	&1	&2	&0	&5	&1	&3	&2\\
\hline
\end{tabular}
\end{table*}



==> tables/tab_result_collated_tr.tex <==
\begin{table*}[t!]
\centering
\small
\caption{Collated best results for SemRe-Rank on all datasets and by all metrics. SSR: SemRe-Rank; s.SSR: supervised SemRe-Rank. Best performing base ATE methods are also shown. We highlight SemRe-Rank scores in\textbf{bold} when they outperform the best performing base ATE methods. }\label{tab_result_collated} 
\begin{tabular}{|l |l l ||l l|}
\hline
Metric     	&\shortstack{SemRe-Rank \\best}	&Configuration	&\multicolumn{2}{|l|}{Best base ATE method}\\
\hline
\multicolumn{5}{|c|}{ACLv2}\\
\hline
P@50	    &\textbf{0.94}	&s.SSR + PU ($m=100$)	&NTM	&0.88\\
P@100	    &\textbf{0.86}	&s.SSR + NTM ($m=100$)/PU ($m=100, 200$)	&PU		&0.85\\
P@500	    &\textbf{0.69}	&s.SSR + CValue ($m=200$)	&NTM/CValue		&0.67\\
P@1000	    &0.60	&SSR/s.SSR + NTM ($m=100,200$)	&NTM	&0.60\\
P@2000	    &0.46	&s.SSR + CValue ($m=100,200$)	&Vote				&0.46\\
%m=500 avgP@K	    &\textbf{.02}	&.\textbf{013}	&\textbf{.003}	&.01	&\textbf{.02}	&\textbf{.02}	&\textbf{.01}	&\textbf{.08}	&\textbf{.09}	&\textbf{.02}	&\textbf{.04}	&\textbf{.03}\\
\hline
Overall P    	&\textbf{0.46}	&s.SSR + CValue ($m=100,200$)	&CValue, Vote		&0.45	\\
Overall R    	&0.54	&SSR/s.SSR with either CValue/TFIDF/Vote ($m=100,200$)	&CValue/TFIDF/Vote				&0.54	\\
Overall F1   	&\textbf{0.50}	&s.SSR + CValue ($m=100,200$)	&CValue/Vote		&0.49	\\
%m=500 Overall (P)    	&.01	&-		&-	&.02	&-				&.01	&.01	&.02			&.02	&	-				&-	&-\\
%m=500 Overall (R)    	&.01	&\textbf{.002}	&-	&.02	&\textbf{.005}	&.01	&.01	&.02			&.03	&	-				&\textbf{.001}	&-\\
%m=500 Overall (F1)   	&.01	&-		&-	&.02	&\textbf{.002}	&.01	&.01	&\textbf{.021}	&.03	&	-				&-	&-\\
\hline
\multicolumn{5}{|c|}{GENIA}\\
\hline
P@50	    &\textbf{0.96}	&SSR/s.SSR + Weirdness ($m=200$)	&GlossEx	&0.88\\
P@100	    &\textbf{0.90}	&SSR/s.SSR + Weirdness ($m=200$)	&CValue		&0.83\\
P@500	    &\textbf{0.82}	&SSR/s.SSR + Weirdness ($m=200$)	&CValue		&0.80\\
P@1000	    &\textbf{0.80}	&s.SSR + Weirdness ($m=100,200$)	&CValue/Vote	&0.78\\
P@2000	    &\textbf{0.78}	&SSR/s.SSR + Weirdness ($m=100,200$)	&TFIDF				&0.77\\
%m=500 avgP@K	    &\textbf{.02}	&.\textbf{013}	&\textbf{.003}	&.01	&\textbf{.02}	&\textbf{.02}	&\textbf{.01}	&\textbf{.08}	&\textbf{.09}	&\textbf{.02}	&\textbf{.04}	&\textbf{.03}\\
\hline
Overall P    	&\textbf{0.54}	&SSR/s.SSR + TFIDF/Weirness ($m=100,200$)	&Weirdness		&0.53	\\
Overall R    	&\textbf{0.66}	&s.SSR + TFIDF ($m=100$)	&TFIDF				&0.63	\\
Overall F1   	&\textbf{0.60}	&s.SSR + TFIDF ($m=100$)	&Weirdness				&0.57	\\%m=500 Overall (P)    	&.01	&-	&-0.02	&-	&-		&.01	&-		&.02	&.01	&.04	&.01	&.01\\
%m=500 Overall (R)    	&\textbf{.012}	&-	&-0.02	&-	&-		&.01	&\textbf{.007}	&.03	&.01	&.03	&.01	&.01\\
%m=500 Overall (F1)   	&\textbf{.011}	&-	&-0.02	&-	&-		&.01	&\textbf{.003}	&.03	&.01	&.04	&.01	&.01\\
\hline
\multicolumn{5}{|c|}{TTCm}\\
\hline
P@50	    &\textbf{0.58}	&s.SSR + TFIDF ($m=200$)	&Basic/CB	&0.52\\
P@100	    &\textbf{0.49}	&s.SSR + CValue ($m=100$)	&PU		&0.39\\
P@500	    &\textbf{0.22}	&s.SSR + CValue ($m=100, 200$)/SSR + CValue ($m=200$)	&CValue		&0.21\\
P@1000	    &0.12	&CValue with any variant of s.SSR/SSR	&CValue	&0.12\\
P@2000	    &0.07	&CValue/TFIDF/$\chi^2$/Vote with any variant of s.SSR/SSR		&CValue/TFIDF/$\chi^2$/Vote				&0.07\\
%m=500 avgP@K	    &\textbf{.02}	&.\textbf{013}	&\textbf{.003}	&.01	&\textbf{.02}	&\textbf{.02}	&\textbf{.01}	&\textbf{.08}	&\textbf{.09}	&\textbf{.02}	&\textbf{.04}	&\textbf{.03}\\
\hline
Overall P    	&\textbf{0.37}	&s.SSR + CValue ($m=200$)	&CValue		&0.33	\\
Overall R    	&\textbf{0.63}	&s.SSR + CValue ($m=200$)	&CValue				&0.55	\\
Overall F1   	&\textbf{0.47}	&s.SSR + CValue ($m=200$)	&CValue				&0.41	\\%m=500 Overall (P)    	&-	&-	&-	&\textbf{.02}	&-		&-0.01	&-	&-	&\textbf{0.00}	&\textbf{0.00}	&\textbf{.03}	&\textbf{0.00}\\
%m=500 Overall (R)    	&-	&-	&-	&\textbf{.03}	&\textbf{.005}		&-0.02	&-	&\textbf{.01}	&\textbf{.01}	&\textbf{0.00}	&\textbf{.04}	&\textbf{0.00}\\
%m=500 Overall (F1)   	&-	&-	&-	&\textbf{.02}	&\textbf{.002}		&-0.01	&-	&-	&\textbf{.004}	&\textbf{0.00}	&\textbf{.03}	&\textbf{0.00}\\
\hline
\multicolumn{5}{|c|}{TTCw}\\
\hline
P@50	    &\textbf{0.54}	&s.SSR + Basic/CB ($m=100$), SSR + Basic ($m=100$)	&Basic/CB/CValue	&0.52\\
P@100	    &\textbf{0.44}	&s.SSR + CValue ($m=100, 200$)	&Basic/CB		&0.41\\
P@500	    &0.16	&s.SSR or SSR + CValue or PU ($m=100,200$)	&PU		&0.16\\
P@1000	    &0.09	&s.SSR or SSR + CValue/PU/Vote ($m=100,200$)	&CValue/PU/Vote	&0.09\\
P@2000	    &0.05	&s.SSR or SSR + CValue/TFIDF/$\chi^2$/PU/Vote ($m=100,200$)	&PU/CValue/$\chi^2$/Vote				&0.05\\
%m=500 avgP@K	    &\textbf{.02}	&.\textbf{013}	&\textbf{.003}	&.01	&\textbf{.02}	&\textbf{.02}	&\textbf{.01}	&\textbf{.08}	&\textbf{.09}	&\textbf{.02}	&\textbf{.04}	&\textbf{.03}\\
\hline
Overall P    	&\textbf{0.28}	&s.SSR + CValue ($m=200$)	&PU		&0.26	\\
Overall R    	&\textbf{0.52}	&s.SSR + CValue ($m=200$)	&PU		&0.50	\\
Overall F1   	&\textbf{0.37}	&s.SSR + CValue ($m=200$)	&PU				&0.34	\\%m=500 Overall (P)    	&-	&-		&-	&-	&-		&-		&-	&-	&-	&-0.01	&.01	&-\\
%m=500 Overall (R)    	&-	&.01	&-	&-	&-		&.01	&-	&-	&-	&-0.03	&.01	&-\\
%m=500 Overall (F1)   	&-	&.003	&-	&-	&-		&.003	&-	&-	&-	&-0.02	&.01	&-\\
\hline
\end{tabular}
\end{table*}



==> tables/tab_result_ptr.tex <==
\begin{table*}[t!]
\centering
\small
\caption{Comparing SemRe-Rank against each base ATE method. Only the difference after re-ranking is shown. () indicates decreased performance. }\label{tab_result_ptr} 
\begin{tabular}{|l |l |l |l|l |l|l||l|l|l|l|l|l|l|l|}
\hline
					&\multicolumn{6}{l||}{ATR4S} 	&\multicolumn{8}{l|}{JATE}\\
\hline
Metric     	&\rotatebox[origin=c]{270}{Basic}	&\rotatebox[origin=c]{270}{\shortstack{Combo\\Basic}}		&\rotatebox[origin=c]{270}{LP}				&\rotatebox[origin=c]{270}{NTM}	&\rotatebox[origin=c]{270}{PU}	&\rotatebox[origin=c]{270}{Voting}			&\rotatebox[origin=c]{270}{CValue}	  &\rotatebox[origin=c]{270}{\shortstack{Gloss-\\Ex}} 	&\rotatebox[origin=c]{270}{RAKE}	&\rotatebox[origin=c]{270}{\shortstack{Rele-\\vance}}	&\rotatebox[origin=c]{270}{TFIDF}	&\rotatebox[origin=c]{270}{\shortstack{Weird-\\ness}}	&\rotatebox[origin=c]{270}{$\chi^{2}$}	&\rotatebox[origin=c]{270}{Voting}\\
\hline
\multicolumn{15}{|c|}{ACLv2}\\
\hline
m=100 changed P@K  	&2	&3	&3	&5	&4	&3	&5	&4	&5	&5	&3	&4	&4	&4\\
m=100 avg diff P@K	    &.02	&.01	&.02	&.01	&.02	&.003	&.01				&.01	&.09	&.09	&.02	&.04	&.02	&.02\\
m=200 changed P@K  	&3	&3	&3	&5	&4	&3	&3	&5	&5	&5	&2	&4	&3	&4\\
m=200 avg diff P@K	    &.02	&.01	&.02	&.01	&.013	&.003	&.012			&.01	&.09	&.11	&.04	&.03	&.02	&.02\\
%m=500 avgP@K	    &.02}	&.013}	&.003}	&.01	&.02}	&.02}	&.01}	&.08}	&.09}	&.02}	&.04}	&.03}\\
\hline
m=100 PRF@K (P)    	&-		&-		&-	&.02	&-	&-				&.01	&.01	&.02			&.01	&	-				&-	&.01	&.01\\
m=100 PRF@K (R)    	&-		&.003	&-	&.02	&.005	&-	&.01	&.01	&.03	&.02	&.002	&-	&.01	&.005\\
m=100 PRF@K (F1)   	&-		&-		&-	&.02	&.002	&-	&.01	&.01	&.03	&.02	&.001	&-	&.01	&.01\\
m=200 PRF@K (P)    	&-		&-		&-	&.02	&-	&-				&.01	&.01	&.02			&.02	&	-				&-	&.01	&.01\\
m=200 PRF@K (R)    	&-		&-		&-	&.02	&.005	&-	&.01	&.01	&.03	&.04	&-	&-	&.01	&.005\\
m=200 PRF@K (F1)   	&-		&-		&-	&.02	&.002	&-	&.01	&.01	&.03	&.03	&	-				&-	&.01	&.01\\
%m=500 PRF@K (P)    	&.01	&-		&-	&.02	&-				&.01	&.01	&.02			&.02	&	-				&-	&-\\
%m=500 PRF@K (R)    	&.01	&.002}	&-	&.02	&.005}	&.01	&.01	&.02			&.03	&	-				&.001}	&-\\
%m=500 PRF@K (F1)   	&.01	&-		&-	&.02	&.002}	&.01	&.01	&.021}	&.03	&	-				&-	&-\\
\hline
\multicolumn{15}{|c|}{GENIA}\\
\hline
m=100 changed P@K  	&4	&4	&5	&5	&2	&5	&5	&4	&5	&5	&3	&5	&5	&3\\
m=100 avg diff P@K	    &.01	&.01	&.05	&.013	&.06	&.01	&.02	&.05	&.06	&.11	&.03	&.08	&.02	&.01\\
m=200 changed P@K  	&4	&4	&5	&5	&2	&5	&5	&4	&5	&5	&3	&5	&5	&5\\
m=200 avg diff P@K	    &.013	&.013	&.04	&.012	&.03	&.01	&.02	&.043	&.06	&.10	&.03	&.08	&.022	&.01\\
%m=500 avgP@K	    &.02}	&.02}	&.04	&.013}	&.02	&.012}	&.04}	&.06}	&.12}	&.033}	&.08	&.022}\\
\hline
m=100 PRF@K (P)    	&.01	&-	&-0.02	&-	&-	&-		&.01	&-		&.03	&.01	&.04	&.01	&.01	&.01\\
m=100 PRF@K (R)    	&.01	&-	&-0.02	&-	&-	&-		&.01	&.007	&.04	&.01	&.033	&.01	&.01	&.005\\
m=100 PRF@K (F1)   	&.01	&-	&-0.02	&-	&-	&-		&.01	&.003	&.04	&.01	&.04	&.01	&.01	&.01\\
m=200 PRF@K (P)    	&.01	&-	&-0.02	&-	&-	&-		&.01	&-		&.03	&.01	&.04	&.01	&.01	&.01\\
m=200 PRF@K (R)    	&.01	&-	&-0.02	&-	&-	&-		&.01	&.007	&.04	&.01	&.03	&.01	&.01	&.005\\
m=200 PRF@K (F1)   	&.01	&-	&-0.02	&-	&-	&-		&.01	&.003	&.04	&.01	&.04	&.01	&.01	&.01\\
%m=500 PRF@K (P)    	&.01	&-	&-0.02	&-	&-		&.01	&-		&.02	&.01	&.04	&.01	&.01\\
%m=500 PRF@K (R)    	&.012}	&-	&-0.02	&-	&-		&.01	&.007}	&.03	&.01	&.03	&.01	&.01\\
%m=500 PRF@K (F1)   	&.011}	&-	&-0.02	&-	&-		&.01	&.003}	&.03	&.01	&.04	&.01	&.01\\
\hline
\multicolumn{15}{|c|}{TTCm}\\
\hline
m=100 changed P@K  	&3	&3	&1	&3	&1	&4	&2	&2	&2	&5	&4	&5	&3	&3\\
m=100 avg diff P@K	    &.01	&.01	&.01	&.01	&(-0.01)	&.01	&.02	&(-0.02)	&.02	&.12	&.04	&.05	&.01	&.02\\
m=200 changed P@K  	&2	&2	&1	&1			&1	&4	&3	&1	&2	&5	&3			&4	&3	&3\\
m=200 avg diff P@K	    &.02	&.02	&.01	&.01	&.01	&.01	&-	&(-0.02)	&.01	&.08	&0.04	&.04	&-	&.01\\
%m=500 avgP@K	    &.02}	&.02}	&.01}	&-	&-	&.03}	&0.01	&.01}	&.03}	&-0.01}	&.01}	&-0.03\\
\hline
m=100 PRF@K (P)    	&-	&-	&-	&.04	&-	&.01		&-	&-	&-	&.09	&.02	&.04	&.01	&-\\
m=100 PRF@K (R)    	&-	&-	&.004	&.07	&-	&.01		&-	&.01	&.01	&.16	&.04	&.05	&.03	&.01\\
m=100 PRF@K (F1)   	&-	&-	&-	&.05	&-	&.01		&-	&.004	&-	&.11	&.03	&.04	&.02	&.004\\
m=200 PRF@K (P)    	&.01	&-	&-	&.02	&-	&.01		&-	&-	&-	&.09	&.03	&.04	&.01	&.01\\
m=200 PRF@K (R)    	&.01	&.004	&.01	&.04	&-	&.01		&.01	&.004	&.01	&.17	&.05	&.06	&.02	&.03\\
m=200 PRF@K (F1)   	&.01	&.002	&-	&.03	&-	&.01		&.004	&.002	&-	&.12	&.04	&.05	&.01	&.02\\
%m=500 PRF@K (P)    	&-	&-	&-	&.02}	&-		&-0.01	&-	&-	&-}	&-}	&.03}	&-}\\
%m=500 PRF@K (R)    	&-	&-	&-	&.03}	&.005}		&-0.02	&-	&.01}	&.01}	&-}	&.04}	&-}\\
%m=500 PRF@K (F1)   	&-	&-	&-	&.02}	&.002}		&-0.01	&-	&-	&.004}	&-}	&.03}	&-}\\
\hline
\multicolumn{15}{|c|}{TTCw}\\
\hline
m=100 changed P@K  	&2	&2	&0	&2	&1	&1	&2	&1	&0	&5	&3	&4	&3	&2\\
m=100 avg diff P@K	   &(-0.02)	 &(-0.02)	&-	&.02	&(-0.01)	&.03	&-	&(-0.02)	&-	&.06	&.03	&.01	&.02	&.03\\
m=200 changed P@K  	&1	&2	&0	&2	&1	&1	&1			&2	&0	&5	&1	&3	&2	&1\\
m=200 avg diff P@K	    &(-0.02)	&-0.01	&-	&.03	&.01	&.02	&.01	&.01	&-	&.04	&.01	&.02	&.01	&.01\\
%m=500 avgP@K	    &-0.01	&-0.01	&-0.01	&-	&-0.01	&.01	&-0.01	&-	&.02	&-	&.01	&-\\
\hline
m=100 PRF@K (P)    	&(-0.01)		&(-0.01)		&-	&.01	&(-0.01)	&-		&.01		&-	&-	&.08	&.02	&.01	&.01	&-\\
m=100 PRF@K (R)    	&(-0.01)		&-	&.02	&.01	&(-0.01)	&-		&.01	&-	&-	&.13	&.04	&.03	&.03	&-\\
m=100 PRF@K (F1)   	&(-0.01)		&(-0.01)	&-	&.01	&(-0.01)	&-		&.01	&-	&-	&.10	&.03	&.02	&.02	&-\\
m=200 PRF@K (P)    	&(-0.01)		&(-0.01)		&-	&.01	&(-0.01)	&.01		&(-0.01)		&-	&-	&.06	&-	&.02	&.01	&-\\
m=200 PRF@K (R)    	&-	&-	&.02	&.01	&(-0.01)	&.01		&(-0.01)	&-	&-	&.10	&.02	&.03	&.03	&-\\
m=200 PRF@K (F1)   	&(-0.005)		&(-0.01)	&-	&.01	&(-0.01)	&.01		&(-0.01)	&-	&-	&.07	&.01	&.02	&.02	&-\\
%m=500 PRF@K (P)    	&-	&-		&-	&-	&-		&-		&-	&-	&-	&-0.01	&.01	&-\\
%m=500 PRF@K (R)    	&-	&.01	&-	&-	&-		&.01	&-	&-	&-	&-0.03	&.01	&-\\
%m=500 PRF@K (F1)   	&-	&.003	&-	&-	&-		&.003	&-	&-	&-	&-0.02	&.01	&-\\
\hline
\end{tabular}
\end{table*}



==> tables/tab_result_ptr_supervised.tex <==
\begin{table*}[t!]
\centering
\small
\caption{Comparing supervised SemRe-Rank against each base ATE method. Only the difference between the two is shown. `-' indicates no change. We also compare results against SemRe-Rank, and use \textbf{Bold} font to indicate that results are better (higher) than the corresponding unsupervised variant, and use (Brackets) indicate that results are worse (lower).}\label{tab_result_ptr_supervised} 
\begin{tabular}{|l |l |l |l|l |l|l||l|l|l|l|l|l|l|l|}
\hline
					&\multicolumn{6}{l||}{ATR4S} 	&\multicolumn{8}{l|}{JATE}\\
\hline
Metric     	&\rotatebox[origin=c]{270}{Basic}				&\rotatebox[origin=c]{270}{\shortstack{Combo\\Basic}}		&\rotatebox[origin=c]{270}{LP}				&\rotatebox[origin=c]{270}{NTM}	&\rotatebox[origin=c]{270}{PU}				&\rotatebox[origin=c]{270}{Voting}	&\rotatebox[origin=c]{270}{CValue}	  &\rotatebox[origin=c]{270}{\shortstack{Gloss-\\Ex}} 	&\rotatebox[origin=c]{270}{RAKE}	&\rotatebox[origin=c]{270}{\shortstack{Rele-\\vance}}	&\rotatebox[origin=c]{270}{TFIDF}	&\rotatebox[origin=c]{270}{\shortstack{Weird-\\ness}}	&\rotatebox[origin=c]{270}{$\chi^{2}$}	&\rotatebox[origin=c]{270}{Voting}\\
\hline
\multicolumn{15}{|c|}{ACLv2}\\
\hline
m=100 changed P@K  	&\textbf{4}	&(2)	&\textbf{4}	&(2)	&\textbf{5}	&4	&(4)	&\textbf{5}	&5	&5	&\textbf{4}	&4	&\textbf{5}	&\textbf{5}\\
m=100 avg diff P@K	    &.02	&\textbf{.03}			&\textbf{.03}	&\textbf{.03}	&\textbf{.04}	&\textbf{.01}	&\textbf{.03}				&.01	&.09	&\textbf{.13}	&\textbf{.07}	&(.03)	&\textbf{.04}	&\textbf{.03}\\
m=200 changed P@K  	&\textbf{4}	&3	&3	&(3)	&\textbf{5}	&3	&\textbf{4}	&(4)	&5	&5	&4	&4	&\textbf{5}	&\textbf{5}\\
m=200 avg diff P@K	    &\textbf{.03}			&\textbf{.02}			&.02	&\textbf{.03}	&\textbf{.04}	&\textbf{.01}	&\textbf{.03}			&\textbf{.02}	&\textbf{.10}	&\textbf{.12}	&\textbf{.09}	&\textbf{.04}	&\textbf{.04}	&\textbf{.03}\\
%m=500 avgP@K	    &\textbf{.02}	&.\textbf{013}	&\textbf{.003}	&.01	&\textbf{.02}	&\textbf{.02}	&\textbf{.01}	&\textbf{.08}	&\textbf{.09}	&\textbf{.02}	&\textbf{.04}	&\textbf{.03}\\
\hline
m=100 PRF@K (P)    	&-		&-		&-	&.02	&-	&-				&(-)	&.01	&\textbf{.03}			&\textbf{.01}	&\textbf{.01}				&-	&.01	&\textbf{.01}\\
m=100 PRF@K (R)    	&.003	&.003	&\textbf{.003}	&.02	&\textbf{.01}	&-	&(-)	&.01	&\textbf{.04}	&\textbf{.03}	&\textbf{.01}	&-	&.01	&\textbf{.01}\\
m=100 PRF@K (F1)   	&-		&-		&-	&.02	&\textbf{.004}	&-	&(-)	&.01	&\textbf{.034}	&.02	&\textbf{.01}	&-	&.01	&\textbf{.01}\\
m=200 PRF@K (P)    	&-		&-		&-	&.02	&-	&-				&.01	&.01	&\textbf{.03}			&.02	&	-				&-	&.01	&\textbf{.01}\\
m=200 PRF@K (R)    	&\textbf{.003}		&\textbf{.003}		&\textbf{.003}	&.02	&\textbf{.01}	&-	&.01	&.01	&\textbf{.04}	&.04	&-	&-	&.01	&\textbf{.01}\\
m=200 PRF@K (F1)   	&-		&-		&-	&.02	&\textbf{.01}	&-	&.01	&.01	&\textbf{.034}	&.03	&	-				&-	&.01	&\textbf{.01}\\
%m=500 PRF@K (P)    	&.01	&-		&-	&.02	&-				&.01	&.01	&.02			&.02	&	-				&-	&-\\
%m=500 PRF@K (R)    	&.01	&\textbf{.002}	&-	&.02	&\textbf{.005}	&.01	&.01	&.02			&.03	&	-				&\textbf{.001}	&-\\
%m=500 PRF@K (F1)   	&.01	&-		&-	&.02	&\textbf{.002}	&.01	&.01	&\textbf{.021}	&.03	&	-				&-	&-\\
\hline
\multicolumn{15}{|c|}{GENIA}\\
\hline
m=100 changed P@K  	&4	&4	&5	&5	&2	&5	&\textbf{5}	&4	&5	&5	&3	&5	&5	&\textbf{4}\\
m=100 avg diff P@K	    &.01	&.01	&.05	&.013	&\textbf{.10}	&.01	&\textbf{.02}	&\textbf{.05}	&\textbf{.06}	&\textbf{.11}	&.03	&.08	&.02	&.01\\
m=200 changed P@K  	&4	&4	&5	&5	&2	&5	&\textbf{5}	&4	&5	&5	&3	&5	&5	&5\\
m=200 avg diff P@K	    &.013	&.013	&\textbf{.053}	&\textbf{.02}	&\textbf{.09}	&.01	&\textbf{.02}	&\textbf{.043}	&\textbf{.06}	&\textbf{.10}	&.03	&.08	&\textbf{.022}	&.01\\
%m=500 avgP@K	    &\textbf{.02}	&\textbf{.02}	&.04	&\textbf{.013}	&.02	&\textbf{.012}	&\textbf{.04}	&\textbf{.06}	&\textbf{.12}	&\textbf{.033}	&.08	&\textbf{.022}\\
\hline
m=100 PRF@K (P)    	&.01	&-	&\textbf{-0.01}	&-	&-	&-		&.01	&-		&\textbf{.03}	&.01	&.04	&.01	&.01	&.01\\
m=100 PRF@K (R)    	&.01	&-	&\textbf{-0.01}	&-	&-	&\textbf{.004}		&.01	&\textbf{.007}	&\textbf{.04}	&.01	&\textbf{.033}	&.01	&.01	&.005\\
m=100 PRF@K (F1)   	&.01	&-	&\textbf{-0.01}	&-	&-	&-		&.01	&\textbf{.003}	&\textbf{.04}	&.01	&.04	&.01	&.01	&.01\\
m=200 PRF@K (P)    	&.01	&-	&\textbf{-0.01}	&-	&-	&-		&.01	&-		&\textbf{.03}	&.01	&.04	&.01	&.01	&.01\\
m=200 PRF@K (R)    	&.01	&-	&\textbf{-0.01}	&-	&-	&\textbf{.004}		&.01	&\textbf{.007}	&\textbf{.04}	&.01	&.03	&.01	&.01	&.005\\
m=200 PRF@K (F1)   	&.01	&-	&\textbf{-0.01}	&-	&-	&-		&.01	&\textbf{.003}	&\textbf{.04}	&.01	&.04	&.01	&.01	&.01\\
%m=500 PRF@K (P)    	&.01	&-	&-0.02	&-	&-		&.01	&-		&.02	&.01	&.04	&.01	&.01\\
%m=500 PRF@K (R)    	&\textbf{.012}	&-	&-0.02	&-	&-		&.01	&\textbf{.007}	&.03	&.01	&.03	&.01	&.01\\
%m=500 PRF@K (F1)   	&\textbf{.011}	&-	&-0.02	&-	&-		&.01	&\textbf{.003}	&.03	&.01	&.04	&.01	&.01\\
\hline
\multicolumn{15}{|c|}{TTCm}\\
\hline
m=100 changed P@K  	&3	&\textbf{4}	&\textbf{1}	&\textbf{5}	&1	&\textbf{4}	&\textbf{3}	&\textbf{3}	&\textbf{3}	&\textbf{5}	&\textbf{4}	&\textbf{5}	&\textbf{3}	&\textbf{4}\\
m=100 avg diff P@K	    &\textbf{.02}	&\textbf{.013}	&\textbf{.01}	&\textbf{.02}	&\textbf{.07}	&\textbf{.02}	&\textbf{.11}	&\textbf{.02}	&.02	&\textbf{.13}	&\textbf{.09}	&.05	&\textbf{.13}	&\textbf{.03}\\
m=200 changed P@K  	&\textbf{4}	&\textbf{4}	&\textbf{3}	&\textbf{5}			&\textbf{3}	&4	&3	&\textbf{3}	&\textbf{5}	&\textbf{5}	&\textbf{4}			&\textbf{5}	&\textbf{4}	&\textbf{4}\\
m=200 avg diff P@K	    &\textbf{.023}	&\textbf{.02}	&\textbf{.013}	&\textbf{.03}	&\textbf{.08}	&\textbf{.013}	&\textbf{0.09}	&\textbf{.01}	&\textbf{.02}	&\textbf{.14}	&\textbf{0.11}	&\textbf{.07}	&\textbf{.14}	&\textbf{.04}\\
%m=500 avgP@K	    &\textbf{.02}	&\textbf{.02}	&\textbf{.01}	&-	&-	&\textbf{.03}	&0.01	&\textbf{.01}	&\textbf{.03}	&\textbf{-0.01}	&\textbf{.01}	&-0.03\\
\hline
m=100 PRF@K (P)    	&-	&-	&-	&\textbf{.05}	&\textbf{.01}	&\textbf{.02}		&-	&\textbf{.01}	&\textbf{.01}	&\textbf{.14}	&\textbf{.03}	&\textbf{.08}	&.01	&\textbf{.02}\\
m=100 PRF@K (R)    	&-	&-	&\textbf{.004}	&\textbf{.08}	&\textbf{.01}	&\textbf{.03}		&-	&.01	&\textbf{.03}	&\textbf{.19}	&\textbf{.07}	&\textbf{.11}	&.03	&\textbf{.05}\\
m=100 PRF@K (F1)   	&-	&-	&-	&\textbf{.06}	&\textbf{.01}	&\textbf{.02}		&-	&\textbf{.01}	&\textbf{.02}	&\textbf{.17}	&\textbf{.04}	&\textbf{.09}	&.02	&\textbf{.03}\\
m=200 PRF@K (P)    	&-	&-	&\textbf{.01}	&\textbf{.06}	&-	&\textbf{.02}		&\textbf{.04}	&-	&\textbf{.01}	&\textbf{.23}	&\textbf{.06}	&\textbf{.11}	&\textbf{.01}	&\textbf{.04}\\
m=200 PRF@K (R)    	&-	&-	&\textbf{.02}	&\textbf{.08}	&-	&\textbf{.03}		&\textbf{.07}	&\textbf{.005}	&\textbf{.02}	&\textbf{.34}	&\textbf{.10}	&\textbf{.13}	&\textbf{.02}	&\textbf{.07}\\
m=200 PRF@K (F1)   	&-	&-	&\textbf{.01}	&\textbf{.07}	&-	&\textbf{.02}		&\textbf{.05}	&.002	&\textbf{.01}	&\textbf{.27}	&\textbf{.047}	&\textbf{.12}	&\textbf{.01}	&\textbf{.05}\\
%m=500 PRF@K (P)    	&-	&-	&-	&\textbf{.02}	&-		&-0.01	&-	&-	&\textbf{0.00}	&\textbf{0.00}	&\textbf{.03}	&\textbf{0.00}\\
%m=500 PRF@K (R)    	&-	&-	&-	&\textbf{.03}	&\textbf{.005}		&-0.02	&-	&\textbf{.01}	&\textbf{.01}	&\textbf{0.00}	&\textbf{.04}	&\textbf{0.00}\\
%m=500 PRF@K (F1)   	&-	&-	&-	&\textbf{.02}	&\textbf{.002}		&-0.01	&-	&-	&\textbf{.004}	&\textbf{0.00}	&\textbf{.03}	&\textbf{0.00}\\
\hline
\multicolumn{15}{|c|}{TTCw}\\
\hline
m=100 changed P@K  	&2	&2	&\textbf{1}	&\textbf{3}	&\textbf{2}	&\textbf{2}	&\textbf{2}	&\textbf{2}	&0	&\textbf{5}	&\textbf{4}	&\textbf{5}	&\textbf{4}	&\textbf{3}\\
m=100 avg diff P@K	    &\textbf{.02}	&\textbf{.02}	&\textbf{.01}	&\textbf{.05}	&\textbf{.11}	&\textbf{.01}	&\textbf{.05}	&\textbf{.02}	&-	&\textbf{.10}	&\textbf{.06}	&\textbf{.03}	&\textbf{.03}	&\textbf{.04}\\
m=200 changed P@K  	&1	&1	&\textbf{2}	&\textbf{3}	&\textbf{2}	&1	&\textbf{3}			&\textbf{2}	&\textbf{1}	&\textbf{5}	&\textbf{4}	&\textbf{5}	&\textbf{4}	&\textbf{3}\\
m=200 avg diff P@K	    &\textbf{.01}	&\textbf{.01}	&\textbf{.01}	&\textbf{.05}	&\textbf{.09}	&\textbf{.03}	&\textbf{.02}	&\textbf{.03}	&\textbf{.01}	&\textbf{.10}	&\textbf{.07}	&\textbf{.03}	&\textbf{.05}	&\textbf{.06}\\
%m=500 avgP@K	    &-0.01	&-0.01	&-0.01	&-	&-0.01	&.01	&-0.01	&-	&.02	&-	&.01	&-\\
\hline
m=100 PRF@K (P)    	&\textbf{0.00}		&\textbf{0.00}		&-	&\textbf{.01}	&\textbf{0.00}	&\textbf{.01}		&\textbf{.02}		&-	&-	&\textbf{.10}	&.02	&\textbf{.04}	&.02	&\textbf{.01}\\
m=100 PRF@K (R)    	&\textbf{.02}	&\textbf{.02}	&.02	&\textbf{.05}	&\textbf{0.00}	&\textbf{.02}		&\textbf{.05}	&-	&-	&\textbf{.16}	&\textbf{.05}	&\textbf{.06}	&\textbf{.05}	&\textbf{.02}\\
m=100 PRF@K (F1)   	&\textbf{.01}	&\textbf{.01}	&-	&\textbf{.01}	&\textbf{0.00}	&\textbf{.01}		&\textbf{.03}	&-	&-	&\textbf{.12}	&.03	&\textbf{.05}	&\textbf{.03}	&\textbf{.01}\\
m=200 PRF@K (P)    	&\textbf{0.00}		&\textbf{0.00}		&-	&\textbf{.03}	&\textbf{0.00}	&\textbf{.02}		&\textbf{.05}		&-	&\textbf{.01}	&\textbf{.15}	&\textbf{.02}	&\textbf{.05}	&\textbf{.01}	&\textbf{.01}\\
m=200 PRF@K (R)    	&\textbf{.02}	&\textbf{.02}	&.02	&\textbf{.053}	&\textbf{0.00}	&\textbf{.04}		&\textbf{.09}	&-	&\textbf{.02}	&\textbf{.27}	&\textbf{.06}	&\textbf{.08}	&\textbf{.03}	&\textbf{.02}\\
m=200 PRF@K (F1)   	&\textbf{.01}	&\textbf{.01}	&-	&\textbf{.04}	&\textbf{0.00}	&\textbf{.02}		&\textbf{.06}	&-	&\textbf{.01}	&\textbf{.19}	&\textbf{.04}	&\textbf{.06}	&\textbf{.02}	&\textbf{.01}\\
%m=500 PRF@K (P)    	&-	&-		&-	&-	&-		&-		&-	&-	&-	&-0.01	&.01	&-\\
%m=500 PRF@K (R)    	&-	&.01	&-	&-	&-		&.01	&-	&-	&-	&-0.03	&.01	&-\\
%m=500 PRF@K (F1)   	&-	&.003	&-	&-	&-		&.003	&-	&-	&-	&-0.02	&.01	&-\\
\hline
\end{tabular}
\end{table*}



==> tables/tab_result_ptr_tr.tex <==
\begin{table*}[t!]
\centering
\small
\caption{Comparing the unsupervised variant of SemRe-Rank against each base ATE method. Only the change after re-ranking is shown. () indicates negative change. }\label{tab_result_ptr} 
\begin{tabular}{|l |l |l |l|l |l|l|l|l|l|l|l|l|l|l|}
\hline
Metric     	&\rotatebox[origin=c]{270}{Basic}	&\rotatebox[origin=c]{270}{\shortstack{Combo\\Basic}}		&\rotatebox[origin=c]{270}{LP}				&\rotatebox[origin=c]{270}{NTM}	&\rotatebox[origin=c]{270}{PU}	&\rotatebox[origin=c]{270}{Vote\textsubscript{5}}			&\rotatebox[origin=c]{270}{CValue}	  &\rotatebox[origin=c]{270}{\shortstack{Gloss-\\Ex}} 	&\rotatebox[origin=c]{270}{RAKE}	&\rotatebox[origin=c]{270}{\shortstack{Rele-\\vance}}	&\rotatebox[origin=c]{270}{TFIDF}	&\rotatebox[origin=c]{270}{\shortstack{Weird-\\ness}}	&\rotatebox[origin=c]{270}{$\chi^{2}$}	&\rotatebox[origin=c]{270}{Vote\textsubscript{7}}\\
\hline
\multicolumn{15}{|c|}{ACLv2}\\
\hline
z=100 chng P@K  	&1		&3		&3		&4		&4		&3		&4		&4		&5		&5		&3		&4		&3		&4\\
z=100 avg P@K	&.03	&.01	&.04	&.01	&.02	&.003	&.003	&.01	&.10	&.09	&.02	&.04	&.03	&.02\\
z=200 chng P@K  	&4		&3		&2		&3		&4		&3		&2		&5		&5		&5		&2		&4		&4		&5\\
z=200 avg P@K	&.02	&.01	&.02	&.01	&.03	&.003	&.02	&.01	&.09	&.10	&.04	&.03	&.02	&.02\\
%z=500 avgP@K	    &.02}	&.013}	&.003}	&.01	&.02}	&.02}	&.01}	&.08}	&.09}	&.02}	&.04}	&.03}\\
\hline
z=100 P@RTP    	&-		&-	&-	&-		&-		&-	&-	&.01	&.02	&.01	&-		&-	&.01	&.01\\
z=100 R@RTP    	&.003	&-	&-	&.04	&.005	&-	&-	&.01	&.02	&.02	&.002	&-	&.01	&.002\\
z=100 F1@RTP   	&-		&-	&-	&.02	&.002	&-	&-	&.01	&.02	&.01	&-		&-	&.01	&.01\\
z=200 P@RTP    	&-		&-	&-	&-		&-		&-	&-	&.01	&.02	&.02	&-		&-	&-		&.02\\
z=200 R@RTP    	&.003	&-	&-	&.04	&.005	&-	&-	&.01	&.02	&.04	&-		&-	&-		&.01\\
z=200 F1@RTP   	&-		&-	&-	&.02	&.002	&-	&-	&.01	&.02	&.03	&-		&-	&-		&.02\\
%z=500 diff ovrl P)    	&.01	&-		&-	&.02	&-				&.01	&.01	&.02			&.02	&	-				&-	&-\\
%z=500 diff ovrl R)    	&.01	&.002}	&-	&.02	&.005}	&.01	&.01	&.02			&.03	&	-				&.001}	&-\\
%z=500 diff ovrl F1)   	&.01	&-		&-	&.02	&.002}	&.01	&.01	&.021}	&.03	&	-				&-	&-\\
\hline
\multicolumn{15}{|c|}{GENIA}\\
\hline
z=100 chng P@K  	&4		&4		&5		&4		&2		&5		&5		&4		&5		&5		&3		&5		&5		&4\\
z=100 avg P@K	&.02	&.02	&.04	&.01	&.02	&.01	&.02	&.05	&.06	&.10	&.03	&.08	&.02	&.003\\
z=200 chng P@K  	&5		&4		&5		&4		&2		&5		&5		&4		&5		&5		&3		&5		&5		&5\\
z=200 avg P@K	&.01	&.02	&.04	&.01	&.05	&.004	&.02	&.05	&.06	&.10	&.03	&.09	&.02	&.01\\
%z=500 avgP@K	    &.02}	&.02}	&.04	&.013}	&.02	&.012}	&.04}	&.06}	&.12}	&.033}	&.08	&.022}\\
\hline
z=100 P@RTP    	&.01	&-	&-	&-	&-	&-		&.01	&-		&.03	&-	&.04	&.01	&.01	&.01\\
z=100 R@RTP    	&.002	&-	&-	&-	&-	&.004	&.01	&.007	&.04	&-	&.04	&.01	&.01	&.004\\
z=100 F1@RTP   	&.01	&-	&-	&-	&-	&-		&.01	&.003	&.04	&-	&.04	&.01	&.01	&.01\\
z=200 P@RTP    	&.004	&-	&-	&-	&-	&-		&-		&-		&.03	&-	&.04	&.01	&.01	&.01\\
z=200 R@RTP    	&.01	&-	&-	&-	&-	&.004	&.01	&.007	&.04	&-	&.04	&.01	&.01	&.004\\
z=200 F1@RTP   	&.01	&-	&-	&-	&-	&-		&.002	&.003	&.04	&-	&.04	&.01	&.01	&.01\\
%z=500 diff ovrl P)    	&.01	&-	&-0.02	&-	&-		&.01	&-		&.02	&.01	&.04	&.01	&.01\\
%z=500 diff ovrl R)    	&.012}	&-	&-0.02	&-	&-		&.01	&.007}	&.03	&.01	&.03	&.01	&.01\\
%z=500 diff ovrl F1)   	&.011}	&-	&-0.02	&-	&-		&.01	&.003}	&.03	&.01	&.04	&.01	&.01\\
\hline
\multicolumn{15}{|c|}{TTCm}\\
\hline
z=100 chng P@K  		&4		&2		&0		&2		&1		&3		&3		&4			&2		&5		&4		&5		&3		&3\\
z=100 avg P@K	    &.01	&.01	&-		&.01	&(.01)&.003	&.01	&-			&.02	&.10	&.04	&.05	&.01	&.02\\
z=200 chng P@K  		&2		&2		&0		&1		&2		&4		&3		&2			&2		&5		&3		&4		&2		&4\\
z=200 avg P@K	    &.03	&.03	&-		&.01	&-		&.01	&-		&(.01)	&.01	&.08	&.04	&.03	&(.01)&.01\\
%z=500 avgP@K	    &.02}	&.02}	&.01}	&-	&-	&.03}	&0.01	&.01}	&.03}	&-0.01}	&.01}	&-0.03\\
\hline
z=100 P@RTP    	&-		&-		&-		&.02	&-	&-		&-		&-		&-		&.08	&.02	&.04	&.01	&-\\
z=100 R@RTP    	&-		&-		&.01	&.04	&-	&-		&.01	&.004	&.01	&.16	&.04	&.05	&.03	&.01\\
z=100 F1@RTP   	&-		&-		&-		&.03	&-	&-		&.002	&-		&-		&.12	&.03	&.04	&.02	&.003\\
z=200 P@RTP    	&-		&-		&-		&.02	&-	&-		&-		&-		&-		&.08	&.03	&.06	&.01	&.01\\
z=200 R@RTP    	&.004	&.004	&.01	&.02	&-	&-		&.01	&-		&.01	&.16	&.05	&.07	&.02	&.02\\
z=200 F1@RTP   	&-		&-		&-		&.02	&-	&-		&.002	&-		&-		&.12	&.04	&.07	&.01	&.01\\
%z=500 diff ovrl P)    	&-	&-	&-	&.02}	&-		&-0.01	&-	&-	&-}	&-}	&.03}	&-}\\
%z=500 diff ovrl R)    	&-	&-	&-	&.03}	&.005}		&-0.02	&-	&.01}	&.01}	&-}	&.04}	&-}\\
%z=500 diff ovrl F1)   	&-	&-	&-	&.02}	&.002}		&-0.01	&-	&-	&.004}	&-}	&.03}	&-}\\
\hline
\multicolumn{15}{|c|}{TTCw}\\
\hline
z=100 chng P@K  		&2			&2		&0	&2		&1			&1		&1		&0	&0	&5		&3		&3		&2		&3\\
z=100 avg P@K	   	&(.02)	&(.02)&-	&.02	&(.01)	&.02	&.01	&-	&-	&.05	&.03	&.02	&.02	&.01\\
z=200 chng P@K  		&2			&1		&0	&2		&1			&1		&1		&1	&0	&5		&1		&2		&1		&1\\
z=200 avg P@K	    &.02		&.01	&-	&.02	&.02		&.02	&.02	&.02&-	&.04	&.01	&.03	&.01	&.01\\
%z=500 avgP@K	    &-0.01	&-0.01	&-0.01	&-	&-0.01	&.01	&-0.01	&-	&.02	&-	&.01	&-\\
\hline
z=100 P@RTP    	&.01		&-			&-		&.01		&-			&-		&.01	&-	&-	&.08	&.01	&.02	&-		&-\\
z=100 R@RTP    	&(.01)		&.004		&-		&.01		&-			&-		&.01	&-	&-	&.14	&.03	&.03	&-		&-\\
z=100 F1@RTP   	&(.01)		&			&-		&.01		&-			&-		&.01	&-	&-	&.10	&.02	&.03	&-		&-\\
z=200 P@RTP    	&-				&-			&-		&.01		&-			&.01	&(.01)&-	&-	&.05	&-		&.02	&.01	&-\\
z=200 R@RTP    	&.01			&.01		&-		&.01		&-			&.01	&(.01)&-	&-	&.09	&.02	&.02	&.01	&-\\
z=200 F1@RTP   	&.003			&.003		&-		&.01		&-			&.01	&(.01)&-	&-	&.06	&.01	&.02	&.01	&-\\
%z=500 diff ovrl P)    	&-	&-		&-	&-	&-		&-		&-	&-	&-	&-0.01	&.01	&-\\
%z=500 diff ovrl R)    	&-	&.01	&-	&-	&-		&.01	&-	&-	&-	&-0.03	&.01	&-\\
%z=500 diff ovrl F1)   	&-	&.003	&-	&-	&-		&.003	&-	&-	&-	&-0.02	&.01	&-\\
\hline
\end{tabular}
\end{table*}



==> tables/tab_result_ptr_tr_supervised.tex <==
\begin{table*}[t!]
\centering
\small
\caption{Comparing the supervised variant of SemRe-Rank against each base ATE method. Only the changes are shown. We also compare results against the unsupervised variant of SemRe-Rank, and use \textbf{Bold} font to indicate that results are better (higher) than the corresponding unsupervised variant, and use (Brackets) indicate that results are worse (lower).}\label{tab_result_ptr_supervised} 
\begin{tabular}{|l |l |l |l|l |l|l|l|l|l|l|l|l|l|l|}
\hline
Metric     	&\rotatebox[origin=c]{270}{Basic}				&\rotatebox[origin=c]{270}{\shortstack{Combo\\Basic}}		&\rotatebox[origin=c]{270}{LP}				&\rotatebox[origin=c]{270}{NTM}	&\rotatebox[origin=c]{270}{PU}				&\rotatebox[origin=c]{270}{Vote\textsubscript{5}}	&\rotatebox[origin=c]{270}{CValue}	  &\rotatebox[origin=c]{270}{\shortstack{Gloss-\\Ex}} 	&\rotatebox[origin=c]{270}{RAKE}	&\rotatebox[origin=c]{270}{\shortstack{Rele-\\vance}}	&\rotatebox[origin=c]{270}{TFIDF}	&\rotatebox[origin=c]{270}{\shortstack{Weird-\\ness}}	&\rotatebox[origin=c]{270}{$\chi^{2}$}	&\rotatebox[origin=c]{270}{Vote\textsubscript{7}}\\
\hline
\multicolumn{15}{|c|}{ACLv2}\\
\hline
z=100 chng P@K  	&\textbf{4}	&3				&3				&(2)			&\textbf{5}	 &\textbf{4}	&4				&\textbf{5}	&5		&5				&\textbf{4}		&4		&\textbf{5}		&4\\
z=100 avg P@K	&(.02)		&\textbf{.013}	&(.03)			&\textbf{.02}	&\textbf{.03}&\textbf{.01}	&\textbf{.03}	&.01		&.10	&\textbf{.13}	&\textbf{.07}	&(.03)	&\textbf{.04}	&.02\\
z=200 chng P@K  	&\textbf{5}	&3				&2				&(2)			&\textbf{5}	&\textbf{4}		&\textbf{4}		&(4)			&5				&5				&\textbf{4}		&4				&\textbf{5}		&5\\
z=200 avg P@K	&.02		&\textbf{.02}	&.02			&\textbf{.04}	&.03		&\textbf{.01}	&\textbf{.03}	&\textbf{.02}	&.09			&\textbf{.12}	&\textbf{.09}	&\textbf{.04}	&\textbf{.04}	&.02\\
%z=500 avgP@K	    &\textbf{.02}	&.\textbf{013}	&\textbf{.003}	&.01	&\textbf{.02}	&\textbf{.02}	&\textbf{.01}	&\textbf{.08}	&\textbf{.09}	&\textbf{.02}	&\textbf{.04}	&\textbf{.03}\\
\hline
z=100 P@RTP   &-		&-		&-	&-		&-				&-		&\textbf{.01}	&.01	&\textbf{.03}		&.01			&\textbf{.01}		&-	&.01	&.01\\
z=100 R@RTP   &.003	&-		&-	&.04	&\textbf{.01}	&-		&\textbf{.002}	&.01	&\textbf{.04}		&\textbf{.03}	&\textbf{.01}		&-	&.01	&.002\\
z=100 F1@RTP  &-		&-		&-	&.02	&\textbf{.003}	&-		&\textbf{.01}	&.01	&\textbf{.03}		&\textbf{.02}	&\textbf{.01}		&-	&.01	&.01\\
z=200 P@RTP   &\textbf{.01}	&-		&-	&-		&\textbf{.01}	&-	&\textbf{.01}	&.01	&\textbf{.03}	&.02	&-	&-	&\textbf{.01}	&(.01)\\
z=200 R@RTP   &.003			&-		&-	&.04	&\textbf{.01}	&-	&\textbf{.002}	&.01	&\textbf{.04}	&.04	&	&-	&\textbf{.01}	&(.002)\\
z=200 F1@RTP  &\textbf{.01}	&-		&-	&.02	&\textbf{.01}	&-	&\textbf{.01}	&.01	&\textbf{.03}	&.03	&-	&-	&\textbf{.01}	&(.01)\\
%z=500 diff ovrl P)    	&.01	&-		&-	&.02	&-				&.01	&.01	&.02			&.02	&	-				&-	&-\\
%z=500 diff ovrl R)    	&.01	&\textbf{.002}	&-	&.02	&\textbf{.005}	&.01	&.01	&.02			&.03	&	-				&\textbf{.001}	&-\\
%z=500 diff ovrl F1)   	&.01	&-		&-	&.02	&\textbf{.002}	&.01	&.01	&\textbf{.021}	&.03	&	-				&-	&-\\
\hline
\multicolumn{15}{|c|}{GENIA}\\
\hline
z=100 chng P@K  	&4		&4		&(4)			&\textbf{5}		&2				&5		&5				&4		&5				&5				&\textbf{4}		&5		&5		&(3)\\
z=100 avg P@K	&(.01)	&.02	&\textbf{.05}	&.01			&\textbf{.09}	&.01	&.02			&.05	&\textbf{.064}	&\textbf{.11}	&\textbf{.04}	&.08	&\textbf{.03}	&\textbf{.01}\\
z=200 chng P@K  	&(4)	&4		&(4)			&\textbf{5}		&2				&5		&5				&4		&5				&5				&\textbf{4}		&5		&5				&5\\
z=200 avg P@K	&\textbf{.02}	&.02	&\textbf{.05}	&.01	&\textbf{.08}	&\textbf{.01}	&.02	&.05	&\textbf{.064}	&\textbf{.12}	&.03			&.09	&\textbf{.03}	&.01\\
%z=500 avgP@K	    &\textbf{.02}	&\textbf{.02}	&.04	&\textbf{.013}	&.02	&\textbf{.012}	&\textbf{.04}	&\textbf{.06}	&\textbf{.12}	&\textbf{.033}	&.08	&\textbf{.022}\\
\hline
z=100 P@RTP    	&.01			&-	&-	&-	&-	&-		&\textbf{.02}	&-		&.03	&-				&.04	&.01	&.01	&.01\\
z=100 R@RTP    	&\textbf{.01}	&-	&-&-	&-	&.004	&\textbf{.02}	&.007	&.04	&-				&.04	&.01	&.01	&\textbf{.01}\\
z=100 F1@RTP   	&.01	&-	&-	&-	&-	&-				&\textbf{.02}	&.003	&.04	&-				&.04	&.01	&.01	&.01\\
z=200 P@RTP    	&\textbf{.01}	&-	&-	&-	&-	&-		&\textbf{.01}	&-		&.03	&\textbf{.01}	&.04	&.01	&.01	&.01\\
z=200 R@RTP    	&.01			&-	&-	&-	&-	&.004	&.01			&.007	&.04	&\textbf{.01}	&.04	&.01	&.01	&\textbf{.01}\\
z=200 F1@RTP   	&.01	&-	&-	&-	&-	&-				&\textbf{.01}	&.003	&.03	&\textbf{.01}	&.04	&.01	&.01	&.01\\
%z=500 diff ovrl P)    	&.01	&-	&-0.02	&-	&-		&.01	&-		&.02	&.01	&.04	&.01	&.01\\
%z=500 diff ovrl R)    	&\textbf{.012}	&-	&-0.02	&-	&-		&.01	&\textbf{.007}	&.03	&.01	&.03	&.01	&.01\\
%z=500 diff ovrl F1)   	&\textbf{.011}	&-	&-0.02	&-	&-		&.01	&\textbf{.003}	&.03	&.01	&.04	&.01	&.01\\
\hline
\multicolumn{15}{|c|}{TTCm}\\
\hline
z=100 chng P@K  	&4	&\textbf{4}	&\textbf{1}	&\textbf{5}	&2	&\textbf{4}	&3	&(3)	&\textbf{3}	&5	&4	&5	&3	&\textbf{4}\\
z=100 avg P@K	    &.01	&.01	&\textbf{.01}	&\textbf{.02}	&\textbf{.08}	&\textbf{.01}	&\textbf{.11}	&\textbf{.02}	&.02	&\textbf{.13}	&\textbf{.09}	&.05	&\textbf{.13}	&\textbf{.03}\\
z=200 chng P@K  	&2	&2	&\textbf{3}	&\textbf{4}			&\textbf{3}	&4	&3	&\textbf{3}	&\textbf{5}	&5	&\textbf{4}			&\textbf{5}	&\textbf{4}	&(3)\\
z=200 avg P@K	    &\textbf{.05}	&\textbf{.04}	&\textbf{.01}	&\textbf{.02}	&\textbf{.08}	&\textbf{.02}	&\textbf{.09}	&\textbf{.01}	&\textbf{.02}	&\textbf{.15}	&\textbf{.10}	&\textbf{.08}	&\textbf{.14}	&\textbf{.04}\\
%z=500 avgP@K	    &\textbf{.02}	&\textbf{.02}	&\textbf{.01}	&-	&-	&\textbf{.03}	&0.01	&\textbf{.01}	&\textbf{.03}	&\textbf{-0.01}	&\textbf{.01}	&-0.03\\
\hline
z=100 P@RTP    	&-	&-	&-	&\textbf{.05}	&\textbf{.01}	&\textbf{.02}		&-	&\textbf{.01}	&\textbf{.01}	&\textbf{.14}	&\textbf{.03}	&\textbf{.08}	&.01	&\textbf{.02}\\
z=100 R@RTP    	&-	&-	&.01	&\textbf{.08}	&\textbf{.01}	&\textbf{.02}		&.01	&\textbf{.01}	&\textbf{.03}	&\textbf{.21}	&\textbf{.06}	&\textbf{.11}	&.03	&\textbf{.05}\\
z=100 F1@RTP   	&-	&-	&-	&\textbf{.06}	&\textbf{.01}	&\textbf{.02}		&.002	&\textbf{.01}	&\textbf{.01}	&\textbf{.17}	&\textbf{.04}	&\textbf{.09}	&.02	&\textbf{.03}\\
z=200 P@RTP    	&-	&-	&\textbf{.01}	&\textbf{.05}	&-	&\textbf{.02}		&\textbf{.04}	&-	&\textbf{.01}	&\textbf{.24}	&\textbf{.05}	&\textbf{.11}	&\textbf{.02}	&\textbf{.04}\\
z=200 R@RTP    	&(-)	&(-)	&\textbf{.02}	&\textbf{.08}	&-	&\textbf{.03}		&\textbf{.08}	&\textbf{.004}	&\textbf{.02}	&\textbf{.35}	&\textbf{.09}	&\textbf{.14}	&\textbf{.03}	&\textbf{.08}\\
z=200 F1@RTP   	&-	&-	&\textbf{.01}	&\textbf{.06}	&-	&\textbf{.02}		&\textbf{.05}	&-	&\textbf{.01}	&\textbf{.28}	&\textbf{.07}	&\textbf{.12}	&\textbf{.03}	&\textbf{.05}\\
%z=500 diff ovrl P)    	&-	&-	&-	&\textbf{.02}	&-		&-0.01	&-	&-	&\textbf{0.00}	&\textbf{0.00}	&\textbf{.03}	&\textbf{0.00}\\
%z=500 diff ovrl R)    	&-	&-	&-	&\textbf{.03}	&\textbf{.005}		&-0.02	&-	&\textbf{.01}	&\textbf{.01}	&\textbf{0.00}	&\textbf{.04}	&\textbf{0.00}\\
%z=500 diff ovrl F1)   	&-	&-	&-	&\textbf{.02}	&\textbf{.002}		&-0.01	&-	&-	&\textbf{.004}	&\textbf{0.00}	&\textbf{.03}	&\textbf{0.00}\\
\hline
\multicolumn{15}{|c|}{TTCw}\\
\hline
z=100 chng P@K  	&2	&2	&\textbf{1}	&\textbf{3}	&\textbf{2}	&\textbf{2}	&\textbf{2}	&\textbf{2}	&0	&\textbf{5}	&\textbf{4}	&\textbf{5}	&\textbf{4}	&3\\
z=100 avg P@K	    &\textbf{.02}	&\textbf{.02}	&\textbf{.01}	&\textbf{.05}	&\textbf{.11}	&\textbf{.01}	&\textbf{.05}	&\textbf{.02}	&-	&\textbf{.10}	&\textbf{.06}	&\textbf{.03}	&\textbf{.03}	&\textbf{.04}\\
z=200 chng P@K  	&2	&1	&\textbf{2}	&\textbf{4}	&\textbf{2}	&1	&\textbf{3}			&\textbf{2}	&\textbf{1}	&\textbf{5}	&\textbf{4}	&\textbf{5}	&\textbf{4}	&\textbf{3}\\
z=200 avg P@K	    &.02	&.01	&\textbf{.01}	&\textbf{.04}	&\textbf{.09}	&\textbf{.03}	&\textbf{.02}	&\textbf{.03}	&\textbf{.01}	&\textbf{.10}	&\textbf{.06}	&.03	&\textbf{.05}	&\textbf{.06}\\
%z=500 avgP@K	    &-0.01	&-0.01	&-0.01	&-	&-0.01	&.01	&-0.01	&-	&.02	&-	&.01	&-\\
\hline
z=100 P@RTP    	&-	&-		&-	&\textbf{.03}	&-	&\textbf{.01}		&\textbf{.02}		&-	&-	&\textbf{.10}	&\textbf{.02}	&\textbf{.04}	&\textbf{.02}	&\textbf{.01}\\
z=100 R@RTP    	&\textbf{.03}	&\textbf{.03}	&\textbf{.02}	&\textbf{.05}	&-	&\textbf{.02}		&\textbf{.04}	&-	&-	&\textbf{.17}	&\textbf{.05}	&\textbf{.06}	&\textbf{.05}	&\textbf{.01}\\
z=100 F1@RTP   	&\textbf{.01}	&\textbf{.01}	&-	&\textbf{.04}	&-	&\textbf{.01}		&\textbf{.03}	&-	&-	&\textbf{.13}	&\textbf{.05}	&\textbf{.05}	&\textbf{.03}	&\textbf{.01}\\
z=200 P@RTP    	&-	&-	&-	&\textbf{.03}	&-	&\textbf{.02}		&\textbf{.05}		&-	&\textbf{.01}	&\textbf{.15}	&\textbf{.02}	&\textbf{.05}	&.01	&\textbf{.01}\\
z=200 R@RTP    	&\textbf{.03}	&\textbf{.02}	&\textbf{.02}	&\textbf{.05}	&-	&\textbf{.03}		&\textbf{.09}	&-	&\textbf{.02}	&\textbf{.27}	&\textbf{.06}	&\textbf{.08}	&\textbf{.03}	&\textbf{.02}\\
z=200 F1@RTP   	&\textbf{.01}	&\textbf{.01}	&-	&\textbf{.04}	&-	&\textbf{.02}		&\textbf{.06}	&-	&\textbf{.01}	&\textbf{.19}	&\textbf{.03}	&\textbf{.06}	&\textbf{.02}	&\textbf{.01}\\
%z=500 diff ovrl P)    	&-	&-		&-	&-	&-		&-		&-	&-	&-	&-0.01	&.01	&-\\
%z=500 diff ovrl R)    	&-	&.01	&-	&-	&-		&.01	&-	&-	&-	&-0.03	&.01	&-\\
%z=500 diff ovrl F1)   	&-	&.003	&-	&-	&-		&.003	&-	&-	&-	&-0.02	&.01	&-\\
\hline
\end{tabular}
\end{table*}



==> tables/tab_result_random.tex <==
\begin{table*}[t!]
\centering
\small
\caption{Comparing RandomRank against each base ATE method. Only the changes are shown. () indicates negative changes. We also highlight cases where RandomRank is performing better the \textit{unsupervised} variant of SemRe-Rank (both $z=100,200$) in \textbf{bold}.}\label{tab_result_random} 
\begin{tabular}{|l |l |l |l |l |l |l|l|l|l|l|l|l|l|l|}
\hline
Metric     	&\rotatebox[origin=c]{270}{Basic}	&\rotatebox[origin=c]{270}{\shortstack{Combo\\Basic}}	&\rotatebox[origin=c]{270}{LP}	&\rotatebox[origin=c]{270}{NTM}	&\rotatebox[origin=c]{270}{PU}	&\rotatebox[origin=c]{270}{Vote\textsubscript{5}}	&\rotatebox[origin=c]{270}{CValue}	  &\rotatebox[origin=c]{270}{\shortstack{Gloss-\\Ex}} 	&\rotatebox[origin=c]{270}{RAKE}	&\rotatebox[origin=c]{270}{\shortstack{Rele-\\vance}}	&\rotatebox[origin=c]{270}{TFIDF}	&\rotatebox[origin=c]{270}{\shortstack{Weird-\\ness}}	&\rotatebox[origin=c]{270}{$\chi^{2}$}	&\rotatebox[origin=c]{270}{Vote\textsubscript{7}}\\
\hline
\multicolumn{15}{|c|}{ACLv2}\\
\hline
chng P@K	    &3		&3		&2		&4		&4		&2	&3		&4		&4		&5		&3		&5		&4		&2\\
avg P@K	    &(.02)	&(.02)	&(.01)	&(.01)	&(.02)		&(.02)	&(.01)	&(.02)	&(.01)	&(.08)	&.02	&(.03)	&(.003)		&-\\
\hline
P@RTP    	&\textbf{.01}	&-	&(.01)	&-	&\textbf{.01}	&-		&-	&-	&-	&(.04)	&.02	&.01		&-		&-\\
R@RTP    	&\textbf{.01}	&-	&(.01)	&-	&-		&-		&-	&-	&-	&(.04)	&(.01)	&-	&-		&(.01)\\
F1@RTP   	&\textbf{.01}	&-	&(.01)	&-	&\textbf{.007}	&-		&-	&-	&-	&(.04)	&.01	&.007	&-		&(.004)\\
\hline
\multicolumn{15}{|c|}{GENIA}\\
\hline
chng P@K		&2		&3	&3		&2		&2		&2		&5	&\textbf{5}	&5	&5	&\textbf{4}	&4	&5		&1\\
avg P@K	    &(.01)	&-	&\textbf{.06}	&\textbf{.03}	&\textbf{.06}	&(.01)	&(.01)	&-	&.01	&(.01)	&.003	&(.01)	&-		&(.01)\\
\hline
P@RTP    	&.01	&-	&\textbf{(.01)}	&-	&\textbf{.01}	&-		&-	&-	&-		&(.04)	&.01	&.01	&-		&-\\
R@RTP    	&.01	&-	&\textbf{(.01)}	&-	&-		&-		&-	&-	&.005	&(.04)	&.01	&-		&-		&-\\
F1@RTP  	&.01	&-	&\textbf{(.01)}	&-	&\textbf{.007}	&-		&-	&-	&-		&(.04)	&.01	&.007	&-		&-\\
\hline
\multicolumn{15}{|c|}{TTCm}\\
\hline
chng P@K		&2		&3	&\textbf{1}		&0	&\textbf{3}		&2		&2		&4	&\textbf{3}		&4		&3		&4		&\textbf{4}		&1\\
avg P@K	    &(.01)	&-	&(.01)	&-	&-		&(.02)	&(.02)		&-	&.02	&.02	&(.02)	&(.01))	&(.03)		&(.02)\\
\hline
P@RTP    	&-		&-	&-		&.02	&(.01)		&(.01)		&(.01)	&.01	&-	&(.01)		&-	&.01	&(.01		&-\\
R@RTP    	&(.004)	&-	&(.02)	&.02	&(.01)		&(.01)		&(.02)	&.004	&-	&-	&(.01)	&-	&-		&-\\
F1@RTP   	&-		&-	&(.01)	&.02	&(.01)		&(.01)		&(.01)	&\textbf{.007}	&-	&(.005)		&-	&.006	&(.01)		&-\\
\hline
\multicolumn{15}{|c|}{TTCw}\\
\hline
chng P@K		&\textbf{3}		&\textbf{3}		&0		&1		&\textbf{3}		&\textbf{2}		&\textbf{2}		&1		&0	&3		&1		&1		&0		&1\\
avg P@K	    &(.01)	&(.01)	&-		&(.02)	&(.05)		&(.01)	&(.02)	&\textbf{.04}	&-	&.02	&(.08)	&(.01)	&-		&.01\\
\hline
P@RTP    	&\textbf{.01}		&\textbf{.01}	&-	&-	&-		&-		&-	&-	&-	&.01	&(.01)	&.01	&-		&(.01)\\
R@RTP    	&.01			&.01	&-	&-	&-		&-		&-	&-	&-	&.02	&(.01)	&.01	&-		&(.01)\\
F1@RTP   	&\textbf{.01}		&\textbf{.01}	&-	&-	&-		&-		&-	&-	&-	&.01	&(.01)	&.01	&-		&(.01)\\
\hline
\end{tabular}
\end{table*}



==> tables/tab_result_textrank.tex <==
\begin{table*}[t!]
\centering
\small
\caption{Comparing modified TextRank against each base ATE method. Only the difference is shown. `-' indicates no change. We also highlight cases where modified TextRank is performing better than the \textit{unsupervised} SemRe-Rank (both $m=100, 200$) in \textbf{bold}.}\label{tab_result_textrank} 
\begin{tabular}{|l |l |l |l |l |l |l||l|l|l|l|l|l|l|l|}
\hline
					&\multicolumn{6}{l||}{ATR4S} 	&\multicolumn{8}{l|}{JATE}\\
\hline
Metric     	&\rotatebox[origin=c]{270}{Basic}	&\rotatebox[origin=c]{270}{\shortstack{Combo\\Basic}}	&\rotatebox[origin=c]{270}{LP}	&\rotatebox[origin=c]{270}{NTM}	&\rotatebox[origin=c]{270}{PU}	&\rotatebox[origin=c]{270}{Voting}	&\rotatebox[origin=c]{270}{CValue}	  &\rotatebox[origin=c]{270}{\shortstack{Gloss-\\Ex}} 	&\rotatebox[origin=c]{270}{RAKE}	&\rotatebox[origin=c]{270}{\shortstack{Rele-\\vance}}	&\rotatebox[origin=c]{270}{TFIDF}	&\rotatebox[origin=c]{270}{\shortstack{Weird-\\ness}}	&\rotatebox[origin=c]{270}{$\chi^{2}$}	&\rotatebox[origin=c]{270}{Voting}\\
\hline
\multicolumn{15}{|c|}{ACLv2}\\
\hline
changed P@K	    &2		&3		&3		&2		&4		&2		&4		&3				&5		&3			&3		&3		&4		&4\\
avg diffP@K	    &-0.02	&-0.01	&.04	&-0.02	&.01	&-0.02	&.01	&\textbf{.03}	&.06	&.02		&.02	&.01	&0.01	&.01\\
\hline
diff PRF@K (P)    	&-	&-		&\textbf{.05}	&-0.02	&-	&-0.01		&.01	&-	&.01	&.01	&-	&.01			&-		&.01\\
diff PRF@K (R)    	&-	&-0.004	&\textbf{.07}	&-0.03	&-	&-0.01		&-		&-	&.02	&.02	&-	&-		&.004	&-\\
diff PRF@K (F1)   	&-	&-		&\textbf{.06}	&-0.02	&-	&-0.01		&.01	&-	&.02	&.01	&-	&.01			&-		&.004\\
\hline
\multicolumn{15}{|c|}{GENIA}\\
\hline
changed P@K		&5		&\textbf{5}		&3				&4				&2		&5		&5		&4			&5		&5				&\textbf{4}		&5		&5		&2\\
avg diffP@K	    &.02	&.02			&\textbf{.06}	&\textbf{.02}	&.05	&.01	&.02	&.03		&.04	&\textbf{.014}	&.03			&.07	&.02	&\textbf{.02}\\
\hline
diff PRF@K (P)    	&-	&-0.01	&-0.01	&-		&-	&-		&\textbf{.02}	&-		&-		&\textbf{.02}	&-	&\textbf{.03}	&-		&.01\\
diff PRF@K (R)    	&-	&-0.006	&-0.01	&-0.004	&-	&-		&\textbf{.03}	&.005	&.005	&\textbf{.03}	&-	&\textbf{.03}	&.003	&.004\\
diff PRF@K (F1)   	&-	&-0.01	&-0.01	&-		&-	&-		&\textbf{.02}	&-		&-		&\textbf{.02}	&-	&\textbf{.03}	&-		&.01\\
\hline
\multicolumn{15}{|c|}{TTCm}\\
\hline
changed P@K		&2		&\textbf{3}		&\textbf{1}		&2				&2				&2		&2			&1		&\textbf{4}		&4		&3	&5		&2				&4\\
avg diffP@K	    &.02	&.01			&\textbf{.01}	&\textbf{.02}	&\textbf{.01}	&-		&-0.01	&-0.02	&.01			&.06	&-	&.02	&\textbf{.02}	&.01\\
\hline
diff PRF@K (P)    	&\textbf{.02}	&\textbf{.02}	&\textbf{.01}	&.02	&-	&\textbf{.01}		&-		&-	&\textbf{.01}	&.05	&.02	&.03	&.01	&.01\\
diff PRF@K (R)    	&\textbf{.02}	&\textbf{.02}	&.01			&.02	&-	&\textbf{.02}		&-		&-	&.01			&.11	&.04	&.04	&.02	&.01\\
diff PRF@K (F1)   	&\textbf{.02}	&\textbf{.02}	&\textbf{.01}	&.02	&-	&\textbf{.01}		&-		&-	&\textbf{.01}	&.07	&.03	&.04	&.01	&.01\\
\hline
\multicolumn{15}{|c|}{TTCw}\\
\hline
changed P@K	    &1		&1		&\textbf{3}		&\textbf{3}		&\textbf{2}		&\textbf{2}			&\textbf{3}		&1		&-		&5				&\textbf{4}		&\textbf{4}		&\textbf{3}			&3\\
avg diffP@K	    &-0.02	&-0.02	&\textbf{.01}	&\textbf{.04}	&\textbf{.04}	&\textbf{.03}		&\textbf{.01}	&.01	&-		&\textbf{0.08}	&\textbf{.04}	&.02			&-					&\textbf{.02}\\
\hline
diff PRF@K (P)    	&\textbf{.01}	&\textbf{.01}	&-				&\textbf{.02}	&-0.01	&-			&.01				&-	&-	&.06	&.01	&\textbf{.03}	&\textbf{.02}	&\textbf{.01}\\
diff PRF@K (R)    	&\textbf{.04}	&\textbf{.04}	&\textbf{.02}	&\textbf{.04}	&-0.01	&.01	&\textbf{.03}	&-	&-	&.11	&.03	&\textbf{.04}	&\textbf{.04}	&\textbf{.01}\\
diff PRF@K (F1)   	&\textbf{.02}	&\textbf{.02}	&-				&\textbf{.03}	&-0.01	&		&\textbf{.02}	&-	&-	&.08	&.02	&.03			&\textbf{.03}	&\textbf{.01}\\
\hline
\end{tabular}
\end{table*}



==> tables/tab_result_tr.tex <==
\begin{table*}[t!]
\centering
\small
\caption{Comparing TermRankStd (standard PageRank) against each base ATE method. Only the difference after TermRank re-ranking is shown. `-' indicates no change.}\label{tab_result_tr} 
\begin{tabular}{|l |l |l |l |l |l|l||l|l|l|l|l|l|l|l|}
\hline
					&\multicolumn{6}{l||}{ATR4S} 	&\multicolumn{8}{l|}{JATE}\\
\hline
Metric     	&\rotatebox[origin=c]{270}{Basic}	&\rotatebox[origin=c]{270}{\shortstack{Combo\\Basic}}	&\rotatebox[origin=c]{270}{LP}	&\rotatebox[origin=c]{270}{NTM}	&\rotatebox[origin=c]{270}{PU}	&\rotatebox[origin=c]{270}{Voting}	&\rotatebox[origin=c]{270}{CValue}	  &\rotatebox[origin=c]{270}{\shortstack{Gloss-\\Ex}} 	&\rotatebox[origin=c]{270}{RAKE}	&\rotatebox[origin=c]{270}{\shortstack{Rele-\\vance}}	&\rotatebox[origin=c]{270}{TFIDF}	&\rotatebox[origin=c]{270}{\shortstack{Weird-\\ness}}	&\rotatebox[origin=c]{270}{$\chi^{2}$}	&\rotatebox[origin=c]{270}{Voting}\\
\hline
\multicolumn{15}{|c|}{ACLv2}\\
\hline
changed P@K	    &4		&3		&2		&2		&4		&?		&2		&4	&5		&5		&2		&4		&3		&?\\
diff avgP@K	    &.01	&.01	&.01	&.01	&.01	&?		&.01	&-	&.07	&.06	&.02	&.02	&.02	&?\\
\hline
diff PRF@K (P)    	&.01	&-	&-	&.02	&-		&?		&.01	&.01	&.02	&.02	&-	&-	&.01	&?\\
diff PRF@K (R)    	&.01	&-	&-	&.02	&.003	&?		&.01	&.01	&.02	&.03	&-	&-	&.01	&?\\
diff PRF@K (F1)   	&.01	&-	&-	&.02	&-		&?		&.01	&.01	&.02	&.03	&-	&-	&.01	&?\\
\hline
\multicolumn{15}{|c|}{GENIA}\\
\hline
changed P@K		&4	&4	&5	&5	&2	&?	&4	&4	&5	&5	&3	&5	&5	&?\\
diff avgP@K	    &.01	&.01	&.04	&.01	&.05	&?		&.01	&.04	&.04	&.09	&.03	&.09	&.02	&?\\
\hline
diff PRF@K (P)    	&.01	&-	&-0.02	&-	&-	&?		&.01	&-		&.02	&.01	&.04	&.01	&.01	&?\\
diff PRF@K (R)    	&.01	&-	&-0.02	&-	&-	&?		&.01	&.004	&.03	&.01	&.03	&.01	&.01	&?\\
diff PRF@K (F1)   	&.01	&-	&-0.02	&-	&-	&?		&.01	&.002	&.03	&.01	&.04	&.01	&.01	&?\\
\hline
\multicolumn{15}{|c|}{TTCm}\\
\hline
changed P@K		&1	&1	&0	&1	&1	&?	&1	&0	&0	&3	&3	&2	&1	&?\\
diff avgP@K	    &-0.04	&-0.04	&-	&-0.01	&.01	&?	&-0.01	&-	&-	&-0.02	&-0.02	&0.01	&-0.02	&?\\
\hline
diff PRF@K (P)    	&-	&-	&-	&-	&-	&?		&-0.01	&-	&-	&-0.04	&-0.01	&.01	&-0.01	&?\\
diff PRF@K (R)    	&-	&-	&-	&-	&-	&?		&-0.02	&-	&-	&-0.04	&-0.03	&.01	&-0.01	&?\\
diff PRF@K (F1)   	&-	&-	&-	&-	&-	&?		&-0.01	&-	&-	&-0.04	&-0.02	&.01	&-0.01	&?\\
\hline
\multicolumn{13}{|c|}{TTCw}\\
\hline
changed P@K		&1	&1	&1	&3	&1	&?	&1	&0	&0	&3	&0	&2	&0	&?\\
diff avgP@K	    &-0.01	&-0.01	&-0.01	&-	&-0.01	&?	&.01	&-0.01	&-	&.02	&-	&.01	&-	&?\\
\hline
diff PRF@K (P)    	&-		&-		&-	&-	&-	&?		&-		&-	&-	&-	&-0.01	&.01	&-	&?\\
diff PRF@K (R)    	&-		&.01	&-	&-	&-	&?		&.01	&-	&-	&-	&-0.03	&.01	&-	&?\\
diff PRF@K (F1)   	&-		&.003	&-	&-	&-	&?		&.003	&-	&-	&-	&-0.02	&.01	&-	&?\\
\hline
\end{tabular}
\end{table*}



==> tables/tab_ttf_precision.tex <==
\begin{table}[t!]
\centering
\small
\caption{Precision of selected seed terms for vector initialization in SemRe-Rank under different $m$.}\label{tab_ttf_precision} 
\begin{tabular}{l | l |l |l |l}
\hline
		   &ACLv2	    &GENIA	&TTCm	&TTCw\\
\hline
\multicolumn{5}{l}{ATR4S}\\
\hline
m=100     	&0.74  	&0.61	&0.32		&0.14\\
m=200	    &0.68	&0.57	&0.24	&0.12\\
\hline
\multicolumn{5}{l}{JATE}\\
\hline
m=100     	&0.63  	&0.65	&0.31		&0.13\\
m=200	    &0.6	&0.69	&0.25	&0.12\\
\hline
\end{tabular}
\end{table}



==> tables/tab_vocab.tex <==
\begin{table}[t!]
\centering
\small
\caption{Vocabulary sizes (both the entire corpus and term candidates extracted by the two libraries) of pre-processed datasets.}\label{tab_vocab} 
\begin{tabular}{l | l |l |l |l }
\hline
				    &ACLv2	&GENIA	&TTCm 	&TTCw \\
\hline
$words(D)$     			&3,920  &19,110 	&20,000	&37,620\\
$words(terms(D))$,ATR4S	&1,922	&7,986	 	&7,086	&11,361\\
$words(terms(D))$,JATE	&2,394 	&10,946		&11,047	&17,037\\
\hline
\end{tabular}
\end{table}



==> tables/tab_vocab_extended.tex <==
\begin{table}[t!]
\centering
\small
\caption{Vocabulary size of pre-processed expanded datasets for training word embedding models. \#unique words - number of unique words in the pre-processed dataset.}\label{tab_vocab_extended} 
\begin{tabular}{l | l |l |l |l }
\hline
Dataset    &ACLv2	&GENIA	&TTCm 	&TTCw \\
\hline
\#unique words     	&21,664  &84,640 	&98,272	&121,668\\
\hline
\end{tabular}
\end{table}

